Improved microgrid resiliency through distributionally robust optimization under a policy-mode framework

Critical energy infrastructure are constantly understress due to the ever increasing disruptions caused by wildfires, hurricanes, other weather related extreme events and cyber-attacks. Hence it becomes important to make critical infrastructure resilient to threats from such cyber-physical events. Such events are however hard to predict and numerous in nature and type, making it infeasible to become resilient to all possible cyber-physical event as such an approach would make the system operation overly conservative. Furthermore, distributions of such events are hard to predict and historical data available on such events is sparse. To deal with these issues, we present a policy-mode framework that enumerates and predicts the probability of various cyber-physical events on top of a distributionally robust optimization (DRO) that is robust to the sparsity of the available historical data. The proposed algorithm is illustrated on an islanded microgrid example: a modified IEEE 123-node feeder with distributed energy resources (DERs) and energy storage.

==> ACC2023_sections/Conclusions.tex <==
This paper presented a Policy-mode framework that based on available risk-predictions of various events, formulates a data-driven distributionally robust optimization (DRO) formulation for a microgrid. Wasserstein ambiguity set framework is utilized to deal with the sparsity in available historical data. Through simulation results we showcase the efficacy of our approach as compared to other probabilistic or risk based methods. 
Future work will look into further reducing the conservativeness of DRO methods and also investigate the applicability of this approach to larger systems (e.g., networked microgrids).

==> ACC2023_sections/DRO_formulation.tex <==
In this Section we will present the Distributionally robust optimization (DRO) formulation that forms the D.R. Optimization block in Fig.~\ref{fig:Event_pred}. Several works in literature including~\cite{duan2018distributionally,zhou2020linear,shi2018distributionally} have used the Wasserstein ambiguity set technique for DRO and this is the DRO technique that will be employed in this work as well. In the next section, we will outline the Wasserstein ambiguity set approach which will then be embedded within the DRO formulation and larger Policy-mode framework.

\subsection{Wasserstein Ambiguity Set}
Here we present an overview of the Wasserstein ambiguity set method for DRO.
In general, the Wasserstein distance between marginal distributions $Q_1$ and $Q_2$ is defined as:

\begin{align}
    W(Q_1,Q_2)=\inf_{\pi}\{\int_{\Xi^2}||\zeta_1-\zeta_2||\pi(d\zeta_1,d\zeta_2)\}
\end{align}
where $\pi$ is the joint distribution of $\zeta_1$ and $\zeta_2$, with marginal distributions $Q_1,Q_2 \in P(\Xi)$.\\
In our case, the Wasserstein distance $W(.,.)$ between the true distribution $\mathbf{P}$ and sample probability distribution $\mathbf{\hat{P}}_N$ is used to define the ambiguity set $\hat{P}_N$ given by:
\begin{align}\label{eq:Wass-exp}
    \hat{P}_N=\{P\in P(\Xi): W(\mathbf{P,\mathbf{\hat{P}}_N}) < \epsilon(N)\}
\end{align}
where $P(\Xi)$ denotes the set of all probability distributions with support $\Xi$ and where:
\begin{align}
    \mathbf{\hat{P}}_N=\frac{1}{N}\sum_{k=1}^N \delta _{\hat{\zeta}^{(k)}}
\end{align}
where $\hat{\zeta}^{(k)} \in \mathbb{R}^N$ are the samples of distribution and $N$ is the number of such samples available. In literature~\cite{duan2018distributionally} the value of $\epsilon(N)$ is usually chosen to be:

\begin{align}
    \epsilon(N)=C\sqrt{\frac{1}{N}log(\frac{1}{1-\beta})}
\end{align}
where $\beta$ is the confidence level of the constraint satisfaction that is required (e.g., $\beta$ = 0.05 when the constraints are required to be satisfied with a 95\% probability).\\
In the above expression, the value of $C$ is calculated as:
\begin{align}
    C\approx \inf_{\alpha >0} (\frac{1}{2\alpha}(1+log(\frac{1}{N}\sum_{k=1}^N e^{\alpha||\hat{\zeta^{(k)}}-\hat{\mu}||^2_1})))^{(1/2)}
\end{align}
where $\hat{\mu}$ is the sample mean and the minimization over $\alpha$ can be solved using the bisection search method. More detailed description about these expressions and how to obtain the search solutions can be found in~\cite{duan2018distributionally}.\\
Based on the above Wasserstein ambiguity set expression in~\eqref{eq:Wass-exp}, the stochastic constraint of the form in~\eqref{eq:CC_Opt}, can be expressed in the DRO form as:
\begin{align}\label{eq:Wass-stoch}
\inf_{\mathbb{P}\in \hat{P}_N} \mathbb{P}[g(x,w)\le 0]\ge 1-\rho
\end{align}
Since the above constraint is intractable, the goal of this section is to develop a convex approximation of~\eqref{eq:Wass-stoch} of the form:
\begin{align}\label{eq:set_U}
    g(x,w)\le 0, \ \forall w \in \mathcal{U}
\end{align}
where $\mathcal{U}$ is a deterministic uncertainty set such that the robust deterministic constraint in~\eqref{eq:set_U} implies satisfaction of the DRO constraint in~\eqref{eq:Wass-stoch}. The rest of the section will focus on finding such a set $U$ that is computationally tractable to obtain.\\
Now, consider the transformation $v=\hat{\Sigma}^{-1/2}(w-\hat{\mu})$, where $\hat{\mu}$ is the sample mean and $\hat{\Sigma}$ is the sample co-variance, which implies that:
\begin{align}
    \mathcal{U}=\hat{\Sigma}^{1/2}\mathcal{V}+\hat{\mu}
\end{align}
Now based on the set $\mathcal{V}$ and considering $Q$ and $Q_N$ to denote the true distribution and empirical distribution of $\mathcal{V}$, the ambiguity set $\hat{Q_N}$, similar to the expression in~\eqref{eq:Wass-exp}, can be obtained as:
\begin{align}
    \sup_{Q\in \hat{Q}_N}Q[v\notin \mathcal{V}]\le \rho
\end{align}
which is now an equivalent representation of the expression in~\eqref{eq:set_U}, where the set $\mathcal{V}$ can now be expressed as:
\begin{align}
    \mathcal{V(\sigma)}=\{v\in \mathbb{R}^m | -\sigma \mathbf{1} < v < \sigma \mathbf{1}\}
\end{align}
where $\sigma$ can be found from solving the optimization problem:
\begin{align}
    \min_{0\leq \lambda, 0 \leq \sigma \leq \sigma_{\text{max}}}\sigma \ s.t. \ h(\sigma,\lambda) \leq \rho
\end{align}
where:
\begin{align}
    h(\sigma, \lambda) = \lambda\epsilon +\frac{1}{N} \sum_{k=1}^N(1-\lambda(\sigma-||\hat{v}^{(k)}||_\infty)^+)+
\end{align}
The above optimization problem can again be solved with the bisection search method as outlined in~\cite{duan2018distributionally}.\\
Based on the solution of $\sigma$, the set $\mathcal{V(\sigma)}$ can be expressed as:
\begin{align}
    \mathcal{V(\sigma)}=Conv(\{\pm \sigma,\pm \sigma\})
\end{align}
where $Conv$ represents the convex combination of the terms.Then the set $\mathcal{U}$ can be expressed as:
\begin{align}
    \mathcal{U}=Conv(\{u^{(1)}, u^{(2)}, \hdots u^{(2m)}\})\\
    u^{(i)}=\hat{\Sigma}^{1/2}\hat{v}^{(i)}+\hat{\mu}, \ 1\leq i \leq 2^m
\end{align}
This results in the following deterministic DRO formulation based on Wasserstein ambiguity set:
\begin{subequations}\label{eq:DRW_Opt}
\begin{align}
&\min_x f(x)\\
\text{s.t.} \ \ &g(x,u^{(i)})\leq 0, \ 1\leq i \leq 2^m
\end{align}
\end{subequations}
where $f$ and $g$ are the objective function and the constraint function respectively as described earlier in~\eqref{eq:Base_Opt}.
Since the set $\mathcal{U}$ can be calculated beforehand, the optimization problem~\eqref{eq:DRW_Opt} can be solved in a scalable manner using off the shelf convex optimization solvers. 
\begin{remark}
\textcolor{blue}{It should be noted that the robustness of the DRO formulation can be tuned through the parameter $\beta$, in a similar manner to the allowable constraint violation parameter $\rho$ in case of CVaR formulation. However, the difference between the two is that DRO accounts for the robustness within the distribution of the disturbance events itself by considering a family of distributions through some metric, whereas CVaR assumes a particular distribution for the disturbance events and only provides performance guarantees within that assumed distribution. The purpose of utilizing DRO for our analysis is to account for the lack of historical data on many of the disturbance events which makes it hard to describe such events completely through a particular distribution. This is the motivation for utilizing a DRO framework in this work. However, DRO can be overly conservative, especially when the possible number of disturbance events are large. This is where the policy-mode framework is able to reduce the dimensionality of considered events by operating the system in one of a certain finite number of operating modes. }
\end{remark}
The next section will provide simulation results on an IEEE-123 node microgrid system that showcases the efficacy of the developed DRO formulation and also compares it with the CVaR formulation.

==> ACC2023_sections/Introduction.tex <==
Critical energy infrastructure has undergone significant changes in the past decades with the increased penetration of distributed energy resources and other inverter-interfaced generation. While this has pushed the goals of green-house gas emission reduction~\cite{di2018decarbonization}, it has also made the energy grid more vulnerable to breakdowns due to the uncertainty and variability in renewable energy generation~\cite{zio2013vulnerability,nazir2019convex}. Furthermore, the risk of weather related outages such as wildfires, hurricanes and other natural disasters have increased in the past years~\cite{NERC2021} and so have the risk of possible cyber-attacks~\cite{HR360}. To deal with the ever increasing challenge posed by such cyber-physical events requires a pivot towards improving the resiliency of our critical energy infrastructure. The US Federal Energy Regulatory Commission (FERC) defines "grid resilience" as the, "Ability to withstand and reduce the magnitude and/or duration of disruptive events, which includes the capability to anticipate, absorb, adapt to, and/or rapidly recover from such an event". 
This work provides a framework for improved resiliency of critical infrastructure systems, with an emphasis on microgrid resiliency. Microgrids are a group of flexible energy resources operating together locally as a single controllable entity~\cite{farrokhabadi2019microgrid}.
In our framework, we assess the risk associated with various cyber-physical events and based on the risk assessment operate the system under a particular policy-mode. This allows us to be resilient against the risks without being overly conservative. Then in order to deal with the sparsity of data available on such cyber-physical events, we develop a distributionally robust optimization (DRO) formulation that is robust to a range of disturbance distributions.

\textbf{Literature review/related work:}
Chance constraints constitute a means to provide certain guarantees on constraint satisfaction under uncertainty~\cite{sahinidis2004optimization} and have found applications in several domains including in power system optimization under uncertainty. The authors in~\cite{dall2017chance} provide a chance constraint formulation for distribution systems with renewable energy resources to enforce voltage regulation with prescribed probability and employ convex approximations of the chance constraints to obtain a computationally tractable formulation. A receding horizon formulation that accounts for the non-linearity in power-flow equations in distribution networks is presented in~\cite{nazir2020stochastic}. Similar chance constraint formulation is utilized for transmission systems in~\cite{roald2017chance}, where a tractable formulation is obtained via partial linearization and a sample based reformulation. A real-time implementation of chance-constrained decision making is provided in~\cite{bolognani2017fast}, where the feasible region of the chance constraint optimization is updated based on real-time measurements. However, a major drawback of chance constraint formulations is that they only consider the probability of constraint violation and not the impact. In many critical infrastructure systems, minimizing the impact of uncertainties is far more significant. Furthermore, many of these methods require assumptions on the probability distribution of the uncertainty and convex reformulations exist only for a very small set of such distributions (e.g., Gaussian), which may not hold in practice.

Distributionally robust chance constraint problems have been well studied in the literature~\cite{calafiore2006distributionally}.
In power systems, to deal with the distributional robustness, the authors in~\cite{summers2015stochastic} consider a family of uncertainty distributions and provide convex reformulations for them. They also consider a conditional value at risk (CVaR) approach that accounts for the risk in constraint violation, as opposed to the probability. Similarly, the authors in~\cite{li2018distributionally} formulate a tractable problem for log-concave distributions and in~\cite{yang2021tractable} the authors formulate a moment based ambiguity set for joint chance constraint formulation, whereas in~\cite{madavan2021stochastic} a primal-dual sub-gradient method is considered to optimize risk constrained optimization problems. Even though, these methods consider the risk in constraint violations, they can often be overly conservative and furthermore still require assumptions on the underlying distribution (e.g., moments) to be accurate.

In case the uncertainty distribution is not known beforehand, sample based approaches have been used in literature~\cite{cheng2019partial}. However, in case of rare events sampling based approaches cannot be applied directly, since they would require an impractical number of samples to yield reasonable solutions~\cite{barrera2016chance}, something which may not be available in practice. To deal with this issue, Wasserstein ambiguity sets have been considered in the literature~\cite{cherukuri2020consistency} where the chance and risk constraints are required to hold for a family of distributions within a distance (Wasserstein distance) from the observed realizations of uncertainty. The Wasserstein-distance based ambiguity set constructed from historical data is applied for solving the OPF problem in~\cite{duan2018distributionally} and a reformulated linearization technique is used to obtain a deterministic LP formulation  in~\cite{zhou2020linear}. In~\cite{guo2018data} the data-driven Wasserstein ambiguity set is utilized to compute control policies in the multi-stage OPF problem. The Wasserstein ambiguity set based DRO is applied to the islanded microgrid case in~\cite{shi2018distributionally} and to the multi-microgrid case in~\cite{huang2020distributionally}.

Even though these methods are distributionally robust, they can be overly conservative in certain situations, especially when there are a large possible number of events and sources of uncertainty present in the system. To deal with the large number of physical events that can disrupt critical infrastructure systems in a manner that is not overly conservative, we formulate a policy-mode based DRO formulation. The policy-mode decides the mode in which the system is operated under from amongst a finite number of modes. The operational policy-mode in turn is decided based on the risk-prediction of various events. Several works in literature have developed risk-based approaches that predict the risk of outages~\cite{kezunovic2022data} and various events such as proactively de-energizing grid components in the context of extreme wildfire risk~\cite{rhodes2020balancing}. Such risk-prediction can often be based upon publicly available data, such as the wildfire risk data from the United States Geological Survey, in case of predicting events such as Public Safety Power Shutoff (PSPS)~\cite{kody2022optimizing}.\\
In this work, we assume the availability of such risk-predictions of various events and then utilize the historical data of such events to formulate a data-driven risk-based DRO formulation for a microgrid. The main advantages of our approach is that it is robust to discrepancies in sampled distribution from historical data by utilizing the Wasserstein ambiguity set, while at the same time avoids being overly conservative by considering the risk-prediction of various events and based on the risk-prediction metrics operate the system under a particular policy-mode considering only a subset of possible events.

\textcolor{blue}{To summarize, the main contributions of this work are enumerated below:
\begin{enumerate}
    \item We present a policy-mode framework that enumerates the various disturbance events, predicts the probability and impact of these events at a given time and then classifies the system operation into a finite number of operational modes to achieve a tractable formulation for dealing with large number of possible disturbance events.
    \item To deal with the sparsity of historical data on such disturbance events, a distributionally robust optimization (DRO) bases formulation using Wasserstein ambiguity balls is utilized within the policy-mode framework to provide guarantees for system security and constraint satisfaction.
    \item The integrated policy-mode framework with the DRO formulation is showcased on an IEEE-distribution system based microgrid and the performance of the algorithms is presented through calculated resilicy metrics.
\end{enumerate}
}

The rest of the paper is organized as follows: Sec.\,II provides the modeling of the microgrid setup and it's various chance constraint and risk constraint formulations. Sec.\,III introduces the Policy-mode framework that considers the risk-prediction of various events and based on these operates the system under a particular policy-mode to avoid being overly conservative. Sec.\,IV presents the distributionally robust formulation that utilizes the Wasserstein ambiguity set framework. Sec.\,V provides the simulation results that showcase the efficacy of the proposed approach and, finally, Sec.\,VI provides conclusions and the scope for future work.

==> ACC2023_sections/Modeling_Formulation.tex <==
\subsection{Baseline optimization}
We consider a microgrid with various distributed energy resources, including solar photovoltaics (PVs), diesel generators (DGs), and energy storage (ES) units. The distribution network power-flow can be expressed by the following linear equations in Branch Flow Model (BFM) format~\cite{gan2014convex}:
\begin{subequations}
\label{eq:pf_linear}
\begin{align}
    0&=W_{n,k}-W_{m,k}+(S_{n,m,k}Z_{n,m}^*+Z_{n,m}S_{n,m,k})\label{eq:P2_volt_rel}\\
0&=\text{diag}(S_{n,m,k})-\sum_{o:m\rightarrow o}\text{diag}(S_{m,o,k})+S^{\text{net}}_{n,k}\label{eq:P2_power_balance}\\
 P^{\text{net}}_{n,k}&=P^\text{pv}_{n,k}+P^\text{dg}_{n,k}+P^\text{es}_{n,k}-P^\text{load}_{n,k} \label{eq:P1_node_real_balance}\\
Q^\text{net}_{n,k}&=Q^\text{pv}_{n,k}+Q^\text{dg}_{n,k}+Q^\text{es}_{n,k}-Q^\text{load}_{n,k}\label{eq:P1_node_reactive_balance}\
\end{align}
\end{subequations}
where: \begin{align*}
    W_{n,k}:=V_{n,k}\cdot V_{n,k}^*\,,\quad I_{n,m,k}:=i_{n,m,k}\cdot i_{n,m,k}^*\,.
\end{align*}
and where $V_{n,k}$ denotes the multi-phase voltage vector at bus $n\in \mathcal{N}$, $i_{n,m,k}$ denotes the multi-phase current flowing from bus $n$ to bus $m$, $S_{n,m,k}$, $P_{n,m,k}$ and $Q_{n,m,k}$ denote the apparent, active and reactive branch power flow from $n\rightarrow m$, $Z_{m,n}$ be the impedance matrix of branch $(n,m)\in \mathcal{L}$, $S_{n,k}^{\text{net}}=P_{n,k}^{\text{net}}+jQ_{n,k}^{\text{net}}$ be the net apparent power injection at bus $n$ and where $\mathcal{N}$ denotes the set of buses, $\mathcal{L}\subset \mathcal{N}\times \mathcal{N}$ denotes the set of all branches and $k$ denotes the time-step. Table  lists the symbols denoting the apparent, active and reactive power associated with each of the energy resources and loads.
\begin{table}[htpb]
    \centering
    \begin{tabular}{c|c|c}
    \hline
         \textsc{apparent, active, reactive} & \textsc{unit} & \textsc{convention}\\
         \hhline{---}
         $\lbrace S_{n,k}^\text{pv}, P_{n,k}^\text{pv}, Q_{n,k}^\text{pv}\rbrace$ & solar PV & injection\\
         $\lbrace S_{n,k}^\text{dg}, P_{n,k}^\text{dg}, Q_{n,k}^\text{dg}\rbrace$ & diesel generator & injection\\
         $\lbrace S_{n,k}^\text{es}, P_{n,k}^\text{es}, Q_{n,k}^\text{es}\rbrace$ & energy storage & injection\\
         $\lbrace S_{n,k}^\text{load},P_{n,k}^\text{load},Q_{n,k}^\text{load}\rbrace$ & load & consumption\\
         \hline
    \end{tabular}
    \caption{Notations used for nodal power exchange}
    \label{tab:notations}
\end{table}
In addition the following operational reliability and safety constraints are imposed:

\begin{subequations}
\label{eq:pf_constraints}
\begin{align}
    &\left|\text{diag}(S_{n,m,k})\right|\leq \overline{S}_{n,m} \label{eq:P1_line_const}\\
&\underline{V}^2\leq \text{diag}(W_{n,k})\leq \overline{V}^2 \label{eq:P1_volt_const}\\
& \left|S^\text{pv}_{n,k}\right|\leq \overline{S}^\text{pv}_n\,,\quad \left|S^\text{dg}_{n,k}\right|\leq \overline{S}^\text{dg}_n\,, \label{eq:gen_constraints}
\end{align}
\end{subequations}
The full description of these constraints and other constraints on battery State-of-charge (SoC) and solar and load curtailment is omitted here for lack of space and can be found in~\cite{nazir2022optimization}. The decision variables in this problem are:
\begin{align*}
    x&:=\left(
    \mathbf{P}_k^\text{pv},\,\mathbf{Q}_k^\text{pv},\mathbf{P}_k^\text{dg},\,\mathbf{Q}_k^\text{dg},\mathbf{P}_k^\text{es},\,\mathbf{Q}_k^\text{es},\mathbf{P}_k^\text{load},\,\mathbf{Q}_k^\text{load}
    \right)
\end{align*}
where the bold-face denotes vectors.

Based on the above equations, the baseline optimization problem for the microgrid can be formulated as:

\begin{subequations}\label{eq:Base_Opt}
\begin{align}
    \min_x f(x)\\
    \text{s.t.} \ \ g(x)\le 0
\end{align}
\end{subequations}
where $x$ denotes the decision variables (e.g., DG dispatch), $f(x)$ is the problem objective (e.g., minimize operating cost) and $g(x)$ are the system constraint (e.g., line limits). An example of the objective function that can be employed here is given by:
\begin{align}
    f(x):=\sum_k \sum_n \left(c_1 \mathbf{P}^\text{dg}_k+c_2 \mathbf{P}^\text{es}_k+c_3 \mathbf{P}^\text{load}_k\right)
\end{align}
The optimization problem in~\eqref{eq:Base_Opt} does not consider uncertainty in system parameters or forecasts, which are critical for practical applications. The next section will consider the optimization problem under uncertainty. 

\subsection{Optimization under uncertainty}
Uncertainty in the system can arise from various adversarial cyber-physical events, like a DG outage, a load-masking attack or a sudden loss in solar generation. In order to be resilient against such events, it is important to have sufficient reserves in the dispatchable resources (DG, PV, storage, and interruptible load) so that these can adjust their output in response to adversarial events. The purpose of this work is to formulate probabilistic methods that determine the amount of reserves requires to deal with such adversarial events in a resilient and cost-effective manner. If we consider a bounded set of uncertainty $w\in \Omega_{\text{W}}$, then the stochastic optimization problem can be expressed as:
\begin{subequations}\label{eq:Stoch_Opt}
\begin{align}
    &\min_x f(x,w)\\
    \text{s.t.} \ \ &g(x,w)\le 0, \ \forall w \in \Omega_{\text{W}}
\end{align}
\end{subequations}
where $x$ also includes additional decision variables in the form of reserves.
However, the above optimization problem is infinite dimensional and cannot be solved in a scalable manner. In the next section, we briefly describe some of the traditional probabilistic methods that are used to solve~\eqref{eq:Stoch_Opt}.
\subsection{Chance constraint formulations}
In this section, we briefly present various stochastic optimization reformulations to solve~\eqref{eq:Stoch_Opt}. One common approach is to robustify~\eqref{eq:Stoch_Opt} against a specified set of adversarial events. In the most general form, the robust optimization problem can be expressed as:

\begin{subequations}\label{eq:arbit_opt}
   \begin{align}
   & \min_{x} \max_{{w}} f({x},w)\\
    s.t. & \ g(x,{w}) \le 0 \qquad \forall {w}\in \Omega_W
\end{align}
\end{subequations}
The above optimization problem can be reformulated using the explicit maximization method, details of which can be found in~\cite{nazir2022optimization,bai2015robust}. However, a robust approach can be overly conservative, especially when the set $w\in \Omega_{\text{W}}$ is large. In such situations, chance constraint based methods can be employed that avoid constraint violation with a certain probability. A general chance constraint optimization can be expressed as:
\begin{subequations}\label{eq:CC_Opt}
\begin{align}
   & \min_x \mathbb{E}[f(x,w)]\\
    \text{s.t.} \ \ & \mathbb{P}[g(x,w)\le 0]\ge 1-\rho
\end{align}
\end{subequations}
\textcolor{blue}{where $\mathbb{E}$ is the expected value operator, $\mathbb{P}$ is the probability operator, and $\rho$ is the pre-specified allowable constraint violation. Chance constraints are closely related to Value at Risk (VaR), a measure used in the finance industry~\cite{rockafellar2000optimization}. Several techniques exist in the literature to obtain tractable reformulations of chance constraints. Most of these methods involve utilizing generating functions that will generate a family of convex approximations for the probabilistic chance constraint~\cite{summers2015stochastic}.
More details about the chance constraint techniques in power systems and their convex reformulations can also be found in~\cite{dall2017chance,roald2017chance}.} \\
One of the main drawbacks of chance constraint methods is that is considers the probability of an event and not the magnitude of constraint violation (risk) of the event. In order to consider the risk of constraint violation, the Conditional value at risk or CVaR method has been employed in the literature~\cite{summers2015stochastic,barrera2016chance}, especially to deal with low probability high impact events, that would otherwise be neglected by the chance constraint formulation, especially for certain types of uncertainty distributions~\cite{rockafellar2000optimization}.Once such CVaR formulation is obtained by from utilizing the Markov generating function. The CVaR based optmization formulation in that case can be expressed as:
\begin{subequations}\label{eq:CVaR_Opt}
\begin{align}
   & \min_x \mathbb{E}[f(x,w)]\\
    \text{s.t.} \ \ & \mathbb{E}[g(x,w) + t]_+\le t\rho
\end{align}
\end{subequations}
% \begin{align}\label{eq:CVaR_Opt}
%     CVaR_{\rho}(w)=\mathbf{E}[w|w\ge VaR_{\rho}(w)]
% \end{align}
where $t$ is an optimization variable and $[.]_+=\max (.,0)$. Further details on the Markov generating functions and other CVaR methods in power systems optimization can be found in~\cite{summers2015stochastic,dall2017chance}.
Even though CVaR related methods account for low probability high impact events, they have an underlying assumption on the probability distribution of the uncertainty, i.e., the historical data used to represent $w \in \Omega_{\text{W}}$ matches the actual distribution. \textcolor{blue}{However, in many practical situations the historical data on adversarial events can be very sparse and hence may not represent the true distribution of such adversarial events. This is a major drawback of chance constraint methods including CVaR that they have an inbuilt assumption on the nature of the probability distribution of the disturbances, an assumption that often breaks down in case of events that have limited historical data. In such cases, distributionally robust optimization (DRO) methods have shown promise~\cite{cherukuri2020consistency,duan2018distributionally}. DRO methods such as the ones based on ambiguity balls consider a family probability distributions within a certain metric in the optimization. By changing the radius of the ambiguity balls, the DRO formulation can be made more robust to lack of sufficient data to represent the disturbance distribution. However, these DRO methods do not deal with the potential conservativeness of such DRO when the adversarial set is large. The contribution of this paper a Policy-mode based framework that reduces the conservativeness of DRO while at the same time accounting for the disturbances in a distributionally robust manner. The Policy-mode based framework achieves this by selecting a subset of disturbance events from a larger pool within a given timeframe based on predicted risks of various disturbance events. In the next section, we present the Policy-mode based framework in detail.}



==> ACC2023_sections/Policy_mode_framework.tex <==
In this section we present a Policy-mode framework implementation for the DRO formulation which is also depicted in Fig.~\ref{fig:Event_pred}. \textcolor{blue}{This framework is one of the main contributions of this paper and presents a mechanism to account for the various disturbances in a way that is not overly conservative. As for many types of disturbances, historical data can be sparse and hence it is difficult to determine the distribution of data for such events. Our policy-mode framework overcomes this limitation through a streamlined process of accounting for various disturbance events while at the same time preventing the solution from becoming overly conservative. The entire framework comprises of four building blocks, each of which will be described in detail in the ensuing text.

\subsection{Scenario Generation}
In the first stage of the framework, shown by the Scenario Generation block in Fig.~\ref{fig:Event_pred}, we enumerate the different events, adversarial attacks, breakdowns, faults and forecast error that can happen in the system and their location. These can be collected based on the history of past events and prediction of possible events that might happen for a system. For the specific microgrid test case that we consider shown in Fig.~\ref{fig:IEEE_123}, we list the various events and their locations in Table~\ref{tab:scenarios}.

\subsection{Event Prediction}
After the scenario generation, the list of possible events collected is passed on to an Event Predictor block. The role of the event predictor is to determine the probability of various events occurring at different locations. The Event Predictor does this based on historical information on the occurrence of these events,  along with the location of their occurrence. Mathematically, the event predictor can be expressed as:

\begin{align}\label{eq:event-predictor}
    \mathbb{P}[event,location]=y(d_i)
\end{align}
where $\mathbb{P}$ is the probability operator, $d_i$ represents the historical data on the events that is used to calculate the probability of events by learning some function $y(.)$.
Examples of methods that could be utilized for such event prediction exist in literature for outages caused by wildfires and other weather related events~\cite{kezunovic2022data,rhodes2020balancing,kody2022optimizing}.
The output of the Event Predictor block is an Event-Location probability matrix that predicts the probability of an event occurring at a particular location as illustrated in Fig.~\ref{fig:Event_pred}. For the microgrid test case, the probability distributions for the considered events is depicted in Fig.~\ref{fig:4dist}, which highlights the heterogeneity amongst different events and why a single distribution cannot be used to represent all of these events.

\subsection{Mode Selection}
After the Event prediction block, the obtained Event Probability matrix is fed into the Mode Selector block. The role of the Mode Selector is to reduce the dimensionality of the problem, as the number of possible events to consider can be very large, making the optimization problem quickly intractable. Here the underlying assumption is that the various events can be grouped together into a mode on the basis that the effect of those events classified within the mode would be same on the system. We consider a certain finite number of modes in which the system operators, where the decision of mode operation is based on simple if then else rules on the Event Probability matrix together with the impact of those events. This can be expressed mathematically as:

\begin{align}\label{eq:mode-selector}
    Mode[i]&=\{1, \ \text{if} \ \mathbb{P}[event[i]]*\mathbb{I}[event[i]] > \mathbb{T}[i]\\
    &=\{0, \ otherwise
\end{align}
where $Mode[i]$ is a binary value representing whether the mode $i$ is operational or not, $\mathbb{I}$ is the impact operator representing the impact (in terms of MWs for the microgrid test-case) on the system due to the event $event[i]$ within the jurisdiction of mode $i$
and finally, $\mathbb{T}[i]$ is the threshold value within the mode $i$ that decides to activate a particular mode or not. As can be seen from~\eqref{eq:mode-selector}, it is possible for multiple modes to be active at the same time, in which case the system would be operator in a mode which accounts for the sum of disturbances within each individual mode.
As an example, Fig.~\ref{fig:Event_pred} lists the modes that the system can operate in and depending upon the values in the Event probability matrix and their impact, the Mode Selector block chooses to operate the system in one or a combination of these modes. For the microgrid test case, the mode selection is based upon the impact of various events at different times as shown in Fig.~\ref{fig:mode-selection}, which can be used to demarcate the time periods into different modes of operation. The reason for using a Mode Selector is to avoid being overly conservative as over a given time horizon only a subset of adversarial events will have significant probability of causing violations in the system constraints.

\subsection{D.R. Optimization}
Finally, the modes of operation along the Event probability matrix is fed to the D.R.Optimization block, that solves a DRO problem and provides resilient operating points and reserves required by the system to operate in a safe manner. Details about the DRO formulation will be provided in the next section.

\begin{figure}[t]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.45\textwidth]{ACC_2023_images/Event-prediction.png}
\caption{\label{fig:Event_pred}Policy mode implementation framework.}
\end{figure}

\begin{figure}[t]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.45\textwidth]{ACC_images/123_modified.png}
\caption{\label{fig:IEEE_123}Modified IEEE-123 node system (from \cite{nazir2022optimization}) with added solar PV, diesel generators and battery units. Note that the bus 76 has collocated diesel and solar generator, while bus 47 has collocated diesel generator and battery.}
\end{figure}

\begin{table}[htpb]
    \centering
    \begin{tabular}{c|c|c}
         \textsc{\#} & \textsc{Events} &  \textsc{Device Location}\\
         \hline\hline
         1 & DG trip & \{47, 49, 65, 76\}\\
         \hline
         2 & PV trip & \{28, 42, 60, 76, 100\}\\
         \hline
         3 & DG cyber-attack & \{47, 49, 65, 76\}\\
         \hline
         4 & PV cyber-attack & \{28, 42, 60, 76, 100\}\\
         \hline
         \multirow{2}{*}{5} & \multirow{2}{*}{Load cyber-attack} & \{1, 6, 28, 29, 35, 42, 47, 48,\\ 
         && 49, 52, 60, 64, 65, 76, 77, 100\}\\
         \hline
         6 & PV forecast error & \{28, 42, 60, 76, 100\}\\
         \hline
         \multirow{2}{*}{7} & \multirow{2}{*}{Load forecast error} & \{1, 6, 28, 29, 35, 42, 47, 48,\\ 
         && 49, 52, 60, 64, 65, 76, 77, 100\}\\
         \hline
         8 & Severe weather PV loss & \{28, 42, 60, 76, 100\}\\
         \hline
         \multirow{2}{*}{9} & \multirow{2}{*}{Severe weather Load loss} & \{1, 6, 28, 29, 35, 42, 47, 48,\\ 
         && 49, 52, 60, 64, 65, 76, 77, 100\}
    \end{tabular}
    \caption{List of events and their locations}
    \label{tab:scenarios}
\end{table}

\begin{figure}[t]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.5\textwidth]{ACC_2023_images/4dist.png}
\caption{\label{fig:4dist}Different distributions of disturbance corresponding to different cyber-physical events.}
\end{figure}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{ACC_2023_images/Impact_modes-new.png}
        \caption{}
        \label{fig:4modes}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=\columnwidth]{ACC_2023_images/Impact_modes-new-2.png}
        \caption{}
        \label{fig:4modes_2}
    \end{subfigure}
    \caption{Impact of various events over time that can be used to decide the mode of system operation}
    \label{fig:mode-selection}
\end{figure*}

==> ACC2023_sections/Simulation_results.tex <==
To illustrate the DRO formulation, we peforms simulations on a modified three-phase IEEE-123 node systems~\cite{kersting2006distribution} shown in Fig.~\ref{fig:IEEE_123}, which is converted into an islanded microgrid by disconnecting the substation from the utility. Table~\ref{tab:scenarios} lists all the possible disturbance events along with their location in the system. These list of scenarios are fed to the Event Predictor block that predicts the probability of various events. Next the Event probability matrix is fed to the Mode Predictor, which based on the impact of different events, decides to operate the system in a particular mode from amongst a finite number of modes. In this case, Fig.~\ref{fig:4modes} and~\ref{fig:4modes_2} shows the impact of the different events over the given time-horizon. Hence based on these figures, Mode Selector chooses to operate the system in Mode 1 (Normal operation) from 0-15 minutes, in Mode 2 (Cyber threat mode) from 15-30 minutes, in Mode 3 (Extreme load loss) from 30-45 minutes and in Mode 4 (Blackout mode) from 45-60 minutes. This mode information along with the impact of different events is next used to solve the DRO formulation.  

We solve the DRO with the event prediction risk probabilities and the forecast of distributions of uncertainty (based on historical data) based on the selected mode of operation. The output of the DRO provides the operating point of the generation and curtailment, along with the reserve values that would be required when the uncertainty reveals itself. It is assumed that the disturbance can be measured through the imbalance in supply and demand which manifests itself in the form of frequency deviation in the system. This frequency measurement is utilized by the flexible resources to dispatch their reserves when the disturbance event occurs~\cite{nazir2022optimization}. To validate the resiliency of the optimization, we perform a series of simulations in GridLab-D~\cite{chassin2008gridlab} by sampling from the true uncertainty distribution. For each sample simulation, the output is calculated as the amount of violation in network constraints (specifically supply-demand imbalance in this case). After running $N$ such simulations from sampled data of the true distribution, we obtain $N$ cases of constraint violations. Based on these $N$ outputs, we next calculate the probability of constraint violation utilizing CVaR metrics~\cite{summers2015stochastic}. The results are validated if the risk of constraint violation from the simulation results is less than the chosen metric in the Wasserstein ambiguity set.\\

In the ideal case, we assume that the sampled distribution (based on historical data) matches the actual distribution of disturbance events as shown in Fig.~\ref{fig:mathched_dist_comp}. In this situation, we apply the CVaR formulation shown in~\eqref{eq:CVaR_Opt} to solve the optimization problem and obtain the operating point and the reserve values. We then sample from the actual distribution to validate the results of the CVaR formulation. As can be seen from Fig.~\ref{fig:CVaR_matched}, in this case the reserves obtained from the CVaR formulation as sufficient (within the chosen 95\% percentile) to manage system resiliency. If on the other hand, the sampled distribution does not match the actual distribution, as depicted in Fig.~\ref{fig:unmatched_dist_comp}, then the assumptions of the CVaR formulation break-down and as a result we observe large constraint violations as depicted in Fig.~\ref{fig:CVaR_unmatched}.\\
Next we apply the DRO formulation based on Wasserstein ambiguity set on the same set of sampled and actual distributions. As seen by the results in Fig.~\ref{fig:DRW_unmatched}, the calculated reserves are able to manage the uncertainty in this case, as it accounts for the disparity between the sampled distribution and actual distribution. However, if the sampled and actual distributions match, then the method may be conservative as depicted in Fig.~\ref{fig:DRW_matched}. Hence, it makes sense to apply the DRO method when there is ambiguity in the available historical data to accurately represent the true distribution of adversarial events. \textcolor{blue}{It should also be pointed out the both the CVaR and DRO formulation can be tuned through parameters ($\rho$ for CVaR and $\beta$ for DRO) to make them more or less conservative. However, the DRO formulation specifically accounts for the mismatch between the assumed distribution of disturbance and the actual distribution of disturbance, whereas the CVaR formulation only increases conservative within the given assumed distribution and hence cannot provide any theoretical guarantees for constraint satisfaction when there is ambiguity with regards to the distribution of uncertainty simply by tuning the parameter $\rho$.} Furthermore, the results in Fig.~\ref{fig:impact_comp_DRW} compare the constraint violation (supply-demand imbalance) between CVaR and DRO in the case when sample distribution is different from actual distribution (Fig.~\ref{fig:unmatched_dist_comp}), which shows the large constraint violation in the CVaR case. Finally, to highlight the trade-off between resiliency (available reserves) and efficiency (inverse of cost), Fig.~\ref{fig:eff_res} shows the trade-off under 4 different modes of operation, when using CVaR in Fig.~\ref{fig:eff_res_CVaR} and when using DRO in Fig.~\ref{fig:eff_res_DRO}, highlighting the larger resiliency in case of DRO but at the cost of lower efficiency. 




% \begin{figure}[htpb]
% \centering
% % \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
% \includegraphics[width=0.4\textwidth]{ACC_2023_images/event_impact.png}
% \caption{\label{fig:4modes}Impact of various events over time that can be used to decide the mode of system operation.}
% \end{figure}







% \begin{figure}[htpb]
% \centering
% % \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
% \includegraphics[width=0.4\textwidth]{ACC_2023_images/event_impact_2.png}
% \caption{\label{fig:4modes_2}Impact of various events over time that can be used to decide the mode of system operation.}
% \end{figure}

% \begin{figure}[htpb]
% \centering
% % \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
% \includegraphics[width=0.4\textwidth]{ACC_2023_images/location_event.png}
% \caption{\label{fig:EL_matrix}Probability of various events over time at different locations.}
% \end{figure}

\begin{figure}[htpb]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.4\textwidth]{ACC_2023_images/matched_dist_comp.png}
\caption{\label{fig:mathched_dist_comp}Comparison of histogram of sampled and actual distribution when they are the same.}
\end{figure}

\begin{figure}[htpb]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.4\textwidth]{ACC_2023_images/CVaR_matched_dist.png}
\caption{\label{fig:CVaR_matched} Disturbance impacts (blue dots) in comparison to available reserves (red lines) when sampled distribution matches actual distribution in CVaR case.}
\end{figure}

\begin{figure}[htpb]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.4\textwidth]{ACC_2023_images/unmatched_dist_comp.png}
\caption{\label{fig:unmatched_dist_comp}Comparison of histograms of sampled and actual distribution when they are different.}
\end{figure}

\begin{figure}[htpb]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.4\textwidth]{ACC_2023_images/CVaR_unmatched_dist.png}
\caption{\label{fig:CVaR_unmatched}Disturbance impacts (blue dots) in comparison to available reserves (red lines) when sampled distribution is different from actual distribution in CVaR case.}
\end{figure}

\begin{figure}[htpb]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.4\textwidth]{ACC_2023_images/DRW_ED.png}
\caption{\label{fig:DRW_unmatched}Disturbance impacts (blue dots) in comparison to available reserves (red lines) when sampled distribution is different from actual distribution in the DRO case.}
\end{figure}

\begin{figure}[htpb]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.4\textwidth]{ACC_2023_images/DRW_ID.png}
\caption{\label{fig:DRW_matched}Disturbance impacts (blue dots) in comparison to available reserves (red lines) when sampled distribution matches actual distribution in the DRO case.}
\end{figure}

\begin{figure}[htpb]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.4\textwidth]{ACC_2023_images/Impact_comp.png}
\caption{\label{fig:impact_comp_DRW}Comparison of the impact of disturbance (mean and variance) over time between CVaR and DRO.}
\end{figure}


\begin{figure*}[htpb]
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{ACC_2023_images/CVaR_eff_res.png}
        \caption{Trade-off between efficiency and resiliency for CVaR}
        \label{fig:eff_res_CVaR}
    \end{subfigure}
    \begin{subfigure}{\columnwidth}
        \centering
        \includegraphics[width=0.8\columnwidth]{ACC_2023_images/DRW_eff_res.png}
        \caption{Trade-off between efficiency and resiliency for DRO}
        \label{fig:eff_res_DRO}
    \end{subfigure}
    \caption{Trade-off between efficiency and resiliency for (a) CVaR (b) DRO.}
    \label{fig:eff_res}
\end{figure*}

==> ACC_sections/AdvSimulations.tex <==
In order to showcase the adversarial set characterization (presented in Sec.\,\ref{sec:adv_set}), we determine the set of largest disturbances which the system can handle. In this scenario we consider losing the largest DG unit, load increase at certain buses, and error in the solar forecast. The baseline optimization problem is solved for each time instant, and given the baseline dispatch, the set $\bar{\Omega}_w$ is computed for each time step by solving $\mathbf{P}_i$ for each potential adversarial event. The maximum component-wise perturbation that can be tolerated and a 2-dimensional projection of $\bar{\Omega}_w$ for specific time instants in shown in Fig \ref{fig:perturbations} and Fig \ref{fig:load_region}. Furthermore, the shape of the set $\bar{\Omega}_w$ changes over time and depends on the amount of flexibility that is available in the system (see Fig \ref{fig:pv1} and Fig \ref{fig:pv2}). Then sampling from the set $\bar{\Omega}_w$ showcases that these disturbances can be handled by the available flexibility. This is shown in Fig.~\ref{fig:CaseCP_Advset} which shows the response of the generators to the loss of DG unit and increase in load and also shows that in this response the SoC constraints are still satisfied. Figure~\ref{fig:CaseCP_Gen} shows that at time $T=20$ minutes there is a loss of DG (chosen randomly between zero and maximum DG loss calculated for the adversarial set). Based on the above analysis, we are guaranteed to have enough reserves available in the system to deal with this disturbance, which can be seen from the increase in battery output and solar PV generation. Furthermore, at $T=30$ minutes, we experience a load increase at certain buses (again chosen randomly at each step between zero and the maximum calculated based on the adversarial set). To deal with this load increase, we dispatch additional flexibility from the battery and the DG units. These simulation results illustrate that the maximum adversarial set calculated in the previous analysis can be managed feasibly by the available flexibility in the microgrid, while maintaining the supply-demand balance and other constraints such as SoC as depicted in Fig.~\ref{fig:CaseCP_SoC}.
\begin{figure}[t]
    \vspace{-9pt}
    \subfloat [\label{fig:perturbations}]{   \includegraphics[width=0.45\linewidth]{ACC_images/perturbations.png}}
    \hfill
  \subfloat[\label{fig:load_region}]{
\includegraphics[width=0.45\linewidth]{ACC_images/load_region.png}}
\caption{Adversarial set characterization: (a) The maximum component-wise perturbation $\alpha_i^\star$ that is supported by the available reserves (b) A 2-dimensional subset of $\bar{\Omega}_w$ for a specific time instant that illustrates the convex region of the tolerable variations in load 1 and 2.}
\end{figure}

\begin{figure}[t]
    \vspace{-9pt}
    \subfloat [\label{fig:pv1}]{   \includegraphics[width=0.45\linewidth]{ACC_images/pv_perturbation1.png}}
    \hfill
  \subfloat[\label{fig:pv2}]{
\includegraphics[width=0.45\linewidth]{ACC_images/pv_perturbation2.png}}
\caption{2-dimensional subset of the time-varying adversarial set $\bar{\Omega}_w$ capturing the allowable variations in solar PV output and load 4, at a) T = 1 minute b) T= 25 min.}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:CaseCP_Gen}]{   \includegraphics[width=0.45\linewidth]{ACC_images/Gen_load_CPcase.png}}
    \hfill
  \subfloat [\label{fig:CaseCP_SoC}]{    \includegraphics[width=0.45\linewidth]{ACC_images/SoC_CPcase.png}}
  \caption{Network constraint under cyber-physical event:(a) Response of the flexible generation under cyber-physical event (b) Battery state of charge (SoC)}
  \label{fig:CaseCP_Advset}
\end{figure}


==> ACC_sections/AdversarialSet.tex <==
While the robust formulation \eqref{eq:robust} can be solved for a given uncertainty set $\Omega_w$\,, it is not known \textit{a priori} what all adversarial events (as specified by the set) the system could be resilient against. In other words, it could be possible that, for a specified adversarial set $\Omega_w$, the problem \eqref{eq:robust} returns infeasible. In this paper, we attempt to address this fact directly by proposing an algorithmic method to characterize the (maximal) adversarial set that the system can tolerate without violation of any critical constraint.

The optimal dispatch $\mathbf{u}^\star$ obtained by solving the optimization problem \eqref{eq:pf_linear}-\eqref{eq:load_curt2} are the set-points associated with the diesel generators, dispatchable loads and solar generation. The goal of the adversarial set characterization is to gain an understanding of the set of adversarial events that can be mitigated by the reserves associated with the optimal dispatch. 
For brevity, we will denote the \textit{robust} version of the constraints \eqref{eq:pf_linear}-\eqref{eq:load_curt2} which jointly considers the decision variables $u \in \mathbb{R}^n$ and the adversarial event $w \in \Omega_W \subset \mathbb{R}^m$  as a convex constraint $g(u, w) \leq 0$.

A polytopic inner approximation $\bar{\Omega}_w$ of $\Omega_w$ that captures the set of adversarial events which can be mitigated by the reserves associated with the optimal dispatch $\mathbf{u}^\star$ can be constructed by solving $m$ optimization problems as follows:
\begin{subequations}
\begin{align}
    \mathbf{P_i:}~ &\max_{w_i}~\alpha_i \\
    &g(\mathbf{u}^\star, w_i) \leq 0\\
    &w_i \in \Omega_w\\
    &w_i = w^{nom} + \alpha_i e_i 
\end{align}
\end{subequations}
%
where $i \in \{1,..m\}$, $e_i \in \mathbb{R}^m$ is the i'th basis vector and $w^{nom}$ is the nominal value of the adversarial disturbance. The nominal value is simply the best  estimate of the adversarial disturbance. In the absence of any information, we can assume that $w_{nom}$ to correspond to the event where there has been no adversarial interference. The optimal solution to $\mathbf{P_i}$ is the vector $w_i^\star$ which maximizes the magnitude of the i'th component of the adversarial vector $w$. We will denote $w_0^\star = w_{nom}$. Since $g$ is convex, it follows that for any convex combination $\sum_{i=1}^m \alpha_i w^\star_i$ of the optimal solutions, $g(\mathbf{u}^\star, \sum_{i=0}^m \alpha_i w^\star_i) \leq 0$. Then, we can define:
\begin{align*}
\bar{\Omega}_w = \{w ~|~ w = \sum_{i=0}^m \alpha_i w_i^\star,~\sum_{i=0}^m \alpha_i = 1, \alpha_i >= 0\}.
\end{align*}
The set $\bar{\Omega}_w$ represents an inner approximation of the set of adversarial events which can be mitigated by the available reserves given that the optimal dispatch is \textit{fixed} to $\mathbf{u}^\star$. 






==> ACC_sections/all_simulation.tex <==
\subsection{Baseline Optimization: Example}
We illustrate the baseline optimization problem \eqref{eq:baseline} on a modified three-phase IEEE-123 node system \cite{kersting2006distribution}, shown in Fig.~\ref{fig:IEEE_123}, which is converted into an islanded microgrid by disconnecting the substation from the utility. The figure shows the location of the solar PV units, diesel generator (DG) units and battery units in the network. {The peak load value in the network is 3.5\,MW (active) and 1.9\,MVAR (reactive). The cumulative maximum generation limit of the DGs is kept at 2.5\,MW, while the cumulative maximum PV generation is 1.77\,MW. The aggregated (charing/discharging) power limit of the batteries is 1.5\,MW, with an aggregated energy capacity of 6\,MWh.} The network model is hosted in GridLAB-D \cite{chassin2008gridlab} and interacts with the baseline optimization (implemented in Julia) via FNCS which is a co-simulation platform  \cite{ciraci2014fncs}. To showcase the baseline optimization problem, we simulate the model under two scenarios: 1) \textit{low solar high load}, and 2) \textit{high solar low load}. 

\begin{figure}[t]
\centering
% \includegraphics[width=0.4\textwidth]{ACC_images/IEEE_123_setup.png}
\includegraphics[width=0.45\textwidth]{ACC_images/123_modified.png}
\caption{\label{fig:IEEE_123}Modified IEEE-123 node system with added solar PV, diesel generators and battery units. Note that the bus 76 has collocated diesel and solar generator, while bus 47 has collocated diesel generator and battery.}
\end{figure}

\subsubsection{Low solar high load case}
This scenario represents the solar and load profiles typically observed during the morning hours, with a low but increasing amount of solar and a high load. The generation and load dispatch for this case is shown in Fig.~\ref{fig:Gen_load_LSHL} which shows how with increasing solar generation over time, the DG generation is reduced in order to reduce the cost of operation. Furthermore, Fig.~\ref{fig:LSHL_curt} shows the curtailment in solar and load, highlighting that initially there a small amount of load curtailment which is required due to inadequate solar PV available, but as the solar PV generation increases, the load curtailment becomes zero. The effect of the generation and load dispatches on the system constraints is depicted in Fig.~\ref{fig:LSHL_output} which shows that the voltages are within their operational limits and the state of charge (SoC) of each battery in the system is also within the SoC limits. In these simulation results, we assume that the initial SoC of the batteries is randomly chosen.

\begin{figure}[t]
\centering
\includegraphics[width=0.3\textwidth]{ACC_images/Gen_load_mor_2.png}
\caption{\label{fig:Gen_load_LSHL} Generation and load in the low solar high load case.}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:solar_curt_LSHL}]{   \includegraphics[width=0.45\linewidth]{ACC_images/solar_comp_mor_2.png}}
    \hfill
  \subfloat [\label{fig:load_curt_LSHL}]{    \includegraphics[width=0.45\linewidth]{ACC_images/load_comp_mor_2.png}}
  \caption{Low solar high load case: (a) Solar curtailment (b) Load curtailment}
  \label{fig:LSHL_curt}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:volt_LSHL}]{   \includegraphics[width=0.45\linewidth]{ACC_images/volt_LSHL.png}}
    \hfill
  \subfloat [\label{fig:SoC_LSHL}]{    \includegraphics[width=0.45\linewidth]{ACC_images/SoC_mor.png}}
  \caption{Low solar high load case: (a) Nodal voltages (b) Battery state of charge evolution.}
  \label{fig:LSHL_output}
\end{figure}

\subsubsection{High solar low load case} 
This scenario represents the solar and load profiles typically observed during the noon/midday hours, with high solar generation but low load. The generation and load dispatch for this case is depicted in Fig.~\ref{fig:Gen_load_HSLL}, which shows how the battery generation reduces and the solar generation increases (since reducing solar curtailment is part of the objective). Also, it can be seen that the DG output is zero as there is sufficient output available from the solar generation and batteries to meet the load. The effect on the system constraints of this generation dispatch is shown in Fig.~\ref{fig:HSLL_output}, which depicts that the voltages are within their nodal limits and that the state of charge (SoC) for all the batteries is within their respective limits (in per unit).

\begin{figure}[t]
\centering
\includegraphics[width=0.3\textwidth]{ACC_images/Gen_load_noon_2.png}
\caption{\label{fig:Gen_load_HSLL} Generation and load in the high solar low load case.}
\end{figure}

%  \begin{figure}[t]
%     %\centering
%     \vspace{-9pt}
%   \subfloat [\label{fig:solar_curt_HSLL}]{   \includegraphics[width=0.45\linewidth]{ACC_images/Solar_curt_HSLL.png}}
%     \hfill
%   \subfloat [\label{fig:load_curt_HSLL}]{    \includegraphics[width=0.45\linewidth]{ACC_images/Load_curt_HSLL.png}}
%   \caption{Case HSLL: (a) Solar curtailment (b) Load curtailment}
%   \label{fig:HSLL_curt}
% \end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:volt_HSLL}]{   \includegraphics[width=0.45\linewidth]{ACC_images/volt_HSLL.png}}
    \hfill
  \subfloat [\label{fig:SoC_HSLL}]{    \includegraphics[width=0.45\linewidth]{ACC_images/SoC_noon.png}}
  \caption{High solar low load case: (a) Nodal voltages (b) Battery state of charge evolution}
  \label{fig:HSLL_output}
\end{figure}

 These case studies show that the baseline optimization satisfies supply-demand balance and is able to satisfy the voltage and state of charge constraints. Furthermore, the amount of load curtailment is minimum and supply is maintained to critical loads in the system.
 
 
 
 
 
 
 
 
 
 
 \subsection{Robust optimization simulation results}

In the following set of simulation results, we will illustrate the effectiveness of the robust formulation (in Sec.\,\ref{sec:verification}). We consider a disturbance event consisting of a cyber-physical event as depicted in Fig.~\ref{fig:CaseCP_DG_trip}, wherein the largest DG in the microgrid (DG 65) trips at time 20\,min and become offline and soon after, at 30\,min, there is a cyber attack which masks the increase in load from the system operator. The DG is made operational and comes back online at 40\,min, whereas the cyber attack is finally over at 50\,min. We solve the robust optimization problem to maintain sufficient reserves in order to meet the increased demand and also maintain system constraints under this cyber-physical event, i.e., the robust optimization problem should have enough reserves to dispatch in case such a cyber-physical event happens on the microgrid. {It is assumed that the disturbance can be measured through the imbalance in supply and demand which manifests itself in the form of frequency deviation in the system. This frequency measurement is utilized by the flexible resources to dispatch their reserves when an adversarial event occurs.} The results for the robust optimization dispatch are shown in Fig.~\ref{fig:CaseCP_agg_gen}. The results show that as the DG trips at 20\,min, the solar PV and the battery increase their output in order meet the load. Furthermore, when the cyber-attack at 30\,min masks the increased load, the battery and PV generation is further increased to meet this load. As the DG unit comes back online and the cyber-attack ends, the battery and solar PV also reduce their output. These simulation results illustrate the effectiveness of the robust formulation to deal with this cyber-physical event. Furthermore, Fig.~\ref{fig:CaseCP_reserve} shows that the robust formulation allocates enough total reserves to deal with this cyber-physical event, i.e., to counter the loss of the largest DG and the load masking cyber-attack. The results in Fig.~\ref{fig:CaseCP_network} demonstrate the effect of this robust dispatch on the system constraints, i.e., the SoC of all the batteries is within their limits and the nodal voltages are within the specified bounds.

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:CaseCP_DG_trip}]{   \includegraphics[width=0.45\linewidth]{ACC_images/CaseCP_DGtrip.png}}
    \hfill
  \subfloat [\label{fig:CaseCP_agg_gen}]{    \includegraphics[width=0.45\linewidth]{ACC_images/CaseCP_Gen_load_2.png}}
  \caption{Cyber-physical event case: (a) DG-trip followed by cyber-attack that masks the increase in load (b) Response of the flexible generation and curtailment to deal with this event}
  \label{fig:Case_CP_event}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.3\textwidth]{ACC_images/CaseCP_reserve_2.png}
\caption{\label{fig:CaseCP_reserve}Supply demand imbalance created by the cyber-physical event and the reserves available to deal with such an event. The figure shows that enough reserves are available to the system operator to effectively deal with this event.}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:CaseCP_SoC1}]{   \includegraphics[width=0.45\linewidth]{ACC_images/CaseCP_SoC_separate.png}}
    \hfill
  \subfloat [\label{fig:CaseCP_volt}]{    \includegraphics[width=0.45\linewidth]{ACC_images/CaseCP_Volt.png}}
  \caption{Network constraint under cyber-physical event: (a) Battery state of charge (SoC) (b) Network voltages}
  \label{fig:CaseCP_network}
\end{figure}


==> ACC_sections/baseline.tex <==
Let us begin by presenting a formulation of the optimal dispatch problem in a microgrid with various distributed energy resources, including solar photovoltaics (PVs), diesel generators (DGs), and energy storage (ES) units. We introduce a few notations for the following mathematical description. Let $\mathcal{N}$ denote the set of all bus indices, and $\mathcal{L}\subseteq\mathcal{N}\times\mathcal{N}$ denote the set of all branches. We use $V_{n,k}$ to denote the multi-phase voltage vector at bus $n\in\mathcal{N}$, at time $k$. The net apparent power injection at bus $n$, at time $k$, is denoted by $S_{n,k}^{\text{net}}=P_{n,k}^{\text{net}}+jQ_{n,k}^{\text{net}}$, where $P_{n,k}^{\text{net}}$ and $Q_{n,k}^{\text{net}}$ are the respective active and reactive power components. Likewise, the Table\,\ref{tab:notations} lists the symbols denoting the apparent, active, and reactive power associated with each of the energy resources and loads at bus $n$, at time $k$\,.
\begin{table}[htpb]
    \centering
    \begin{tabular}{c|c|c}
    \hline
         \textsc{apparent, active, reactive} & \textsc{unit} & \textsc{convention}\\
         \hhline{---}
         $\lbrace S_{n,k}^\text{pv}, P_{n,k}^\text{pv}, Q_{n,k}^\text{pv}\rbrace$ & solar PV & injection\\
         $\lbrace S_{n,k}^\text{dg}, P_{n,k}^\text{dg}, Q_{n,k}^\text{dg}\rbrace$ & diesel generator & injection\\
         $\lbrace S_{n,k}^\text{es}, P_{n,k}^\text{es}, Q_{n,k}^\text{es}\rbrace$ & energy storage & injection\\
         $\lbrace S_{n,k}^\text{load},P_{n,k}^\text{load},Q_{n,k}^\text{load}\rbrace$ & load & consumption\\
         \hline
    \end{tabular}
    \caption{Notations used for nodal power exchange}
    \label{tab:notations}
\end{table}
%
%
Let $E_{n,k}^\text{es}$ be the storage state of charge (SoC). Furthermore, let $i_{n,m,k}$ be the complex vector denoting the multi-phase current flowing from bus $n$ to bus $m$ (i.e., $n\rightarrow m$), at time $k$. Let $S_{n,m,k},\,P_{n,m,k}$ and $Q_{n,m,k}$ denote, respectively, the apparent, active, and reactive branch power-flow from $n\rightarrow m$\,, at time $k$\,. Let $Z_{n,m}\!=\!Z_{m,n}$ be the impedance matrix of the branch $(n,m)\!\in\!\mathcal{L}$. Furthermore, we define (with $\left(\cdot\right)^*$ denoting conjugate transpose):
\begin{align*}
    W_{n,k}:=V_{n,k}\cdot V_{n,k}^*\,,\quad I_{n,m,k}:=i_{n,m,k}\cdot i_{n,m,k}^*\,.
\end{align*}

% Also let $S^{\text{G}}_{n,k}=P^{\text{G}}_{n,k}+jq^{\text{G}}_{n,k}$ be the complex power from the diesel generator and let $P^{\text{Lc}}_{n,k}, Q^{\text{Lc}}_{n,k}$ be the load curtailment and 
% $P^{\text{Sc}}_{n,k}$ be the solar curtailment. 

The distribution network power-flow equations can be expressed in the Branch Flow Model (BFM) \cite{gan2014convex} as:
\begin{subequations}
\label{eq:pf_bfm}
\begin{align}
\begin{bmatrix}
W_{n,k} & S_{n,m,k}\\
S_{n,m,k}^{*} & I_{n,m,k}\end{bmatrix}=
\begin{bmatrix}
V_{n,k}\\
i_{n,m,k}\end{bmatrix}
\begin{bmatrix}
V_{n,k}\\
i_{n,m,k}\end{bmatrix}^{*} &\label{eq:P1_BFM}\\
W_{n,k}=W_{m,k}-(S_{n,m,k}Z_{n,m}^*+Z_{n,m}S_{n,m,k})&\notag\\
+Z_{n,m}I_{n,m,k}Z_{n,m}^*&\label{eq:P1_volt_rel}\\
\!\!S^{\text{net}}_{n,k}+\text{diag}(S_{n,m,k}\!-\!Z_{n,m} I_{n,m,k})=\!\!\!\sum_{o:m\rightarrow o}\!\!\!\text{diag}( S_{m,o,k})& \label{eq:P1_power_balance}
\end{align}
\end{subequations}
The nonlinearity of the power-flow equations in \eqref{eq:pf_bfm} render the resulting optimal dispatch problem non-convex (and NP-hard). While convex relaxations of the power-flow have been proposed in the literature (see \cite{nazir2020optimal} and the references therein), in this paper, we adopt a linearized power-flow model which typically yields acceptable solutions \cite{bolognani2015fast}. In particular, the linearized BFM model \cite{gan2014convex} is given as below:
\begin{subequations}
\label{eq:pf_linear}
\begin{align}
    0&=W_{n,k}-W_{m,k}+(S_{n,m,k}Z_{n,m}^*+Z_{n,m}S_{n,m,k})\label{eq:P2_volt_rel}\\
0&=\text{diag}(S_{n,m,k})-\sum_{o:m\rightarrow o}\text{diag}(S_{m,o,k})+S^{\text{net}}_{n,k}\label{eq:P2_power_balance}
\end{align}
\end{subequations}
%
Next, based on the convention in Table\,\ref{tab:notations}, the net active and reactive power injections at each bus $n$ satisfy the relations:
\begin{subequations}
\begin{align}
    P^{\text{net}}_{n,k}&=P^\text{pv}_{n,k}+P^\text{dg}_{n,k}+P^\text{es}_{n,k}-P^\text{load}_{n,k} \label{eq:P1_node_real_balance}\\
Q^\text{net}_{n,k}&=Q^\text{pv}_{n,k}+Q^\text{dg}_{n,k}+Q^\text{es}_{n,k}-Q^\text{load}_{n,k}\label{eq:P1_node_reactive_balance}\
\end{align}
\end{subequations}

The power system operational reliability and safety dictate imposing certain constraints on the bus voltages and the line flows, as follows:
\begin{subequations}
\label{eq:pf_constraints}
\begin{align}
    &\left|\text{diag}(S_{n,m,k})\right|\leq \overline{S}_{n,m} \label{eq:P1_line_const}\\
&\underline{V}^2\leq \text{diag}(W_{n,k})\leq \overline{V}^2 \label{eq:P1_volt_const}
\end{align}
\end{subequations}
where $\underline{V}$ and $\overline{V}$ are, respectively, the maximum and minimum allowable voltage limits (e.g., specified by ANSI C84.1 Standard), while $\overline{S}_{n,m}$ is the maximum limit on the line-flow.

The inequality constraints that govern the solar PV and diesel power generation is given by the following:
% \begin{subequations}
% \begin{align}
%     &(P^{\text{S}}_{n,k}-P^{\text{Sc}}_{n,k})^2+(Q^{\text{S}}_{n,k})^2\leq G_{\text{max},n}^2 \label{eq:P1_solar_inv_limit}\\
% &|S^{\text{G}}_{n,k}|\leq D_{\text{max},n} \label{eq:P1_diesel_inv_limit}
% \end{align}
% \label{eq:gen_constraints}
% \end{subequations}
\begin{align}
\left|S^\text{pv}_{n,k}\right|\leq \overline{S}^\text{pv}_n\,,\quad \left|S^\text{dg}_{n,k}\right|\leq \overline{S}^\text{dg}_n\,, \label{eq:gen_constraints}
\end{align}
where $\overline{S}^\text{pv}_n$ denotes the inverter capacity at bus $n$, and $\overline{S}^\text{dg}_n$ is the rated size of the diesel generator at bus $n$.

Finally, the energy storage units are associated with a state-of-charge (SoC) dynamics, as well as limits on the charging/discharging rates, limits on the SoC (i.e., storage size), and the inverter capacity, as follows:
\begin{subequations}\label{eq:es_constraints}
\begin{align}
E_{n,k+1}^\text{es}&=E_{n,k}^\text{es}-P^\text{es}_{n,k}\Delta t \label{eq:P1_battery_power_rel}\\
\quad \underline{E}_n^\text{es} &\leq E_{n,k}^\text{es}\leq \overline{E}_n^\text{es} \label{eq:P1_SOC_limit}\\
-\overline{P}_n^\text{es} &\leq P^\text{es}_{n,k}\leq \overline{P}_n^\text{es} \label{eq:P1_Pd_limit}\\
\left|S^\text{es}_{n,k}\right|&=\sqrt{(P^\text{es}_{n,k})^2+(Q^\text{es}_{n,k})^2}\leq \overline{S}^\text{es}_n \label{eq:P1_battery_inv_limit}
\end{align}
\end{subequations}
where $\overline{P}^\text{es}_n$ is the maximum absolute limit on charging (and discharging power), while $\overline{E}^\text{es}_n$ and $\underline{E}^\text{es}_n$ are the respective maximum and minimum limits of SoC. The storage inverter capacity is denoted by $\overline{S}^\text{es}_n$\,.

The decision variables (i.e., dispatchable quantities) considered in this work are:
\begin{align*}
    u&:=\left(
    \mathbf{P}_k^\text{pv},\,\mathbf{Q}_k^\text{pv},\mathbf{P}_k^\text{dg},\,\mathbf{Q}_k^\text{dg},\mathbf{P}_k^\text{es},\,\mathbf{Q}_k^\text{es},\mathbf{P}_k^\text{load},\,\mathbf{Q}_k^\text{load}
    \right)
\end{align*}
where the bold-faced $\mathbf{P}_k^\text{pv}=\left[P^\text{pv}_{n,k}\right]$ denotes the vector of the solar active power variables at all buses, at time $k$, and likewise for the rest. The following additional physical constraints are placed on the solar and load dispatch.
\begin{itemize}
    \item \textit{Solar curtailment}: In a predictive optimization setting, we assume the availability of solar forecast $\widehat{P}^\text{pv}_{n,k}$\,, such that the dispatched solar active power should satisfy
    \begin{align}\label{eq:pv_curt1}
        0\leq {P}^\text{pv}_{n,k}\leq \widehat{P}^\text{pv}_{n,k}\,.
    \end{align}
    Any available solar not dispatched is henceforth referred to as the solar curtailment:
    \begin{align}\label{eq:pv_curt2}
    {P}^\text{pv,curt}_{n,k}:=\widehat{P}^\text{pv}_{n,k}    -{P}^\text{pv}_{n,k}\,.
    \end{align}
    
    \item \textit{Load curtailment}: We assume that each load bus, the \textit{desired}, $P^\text{load,des}_{n,k}$\,, and \textit{minimum (critically necessary)}, $P^\text{load,min}_{n,k}$\,, load values are specified/available. Therefore the dispatched load value should follow certain limits:
    \begin{align}\label{eq:load_curt1}
        P^\text{load,min}_{n,k}\leq P^\text{load}_{n,k}\leq P^\text{load,des}_{n,k}\,.
    \end{align}
    Typically, the range of specified flexibility is narrower for critical loads for which the specified minimum value would be close to (or, same as) the desired value. Any unmet load is referred to as load curtailment:
    \begin{align}\label{eq:load_curt2}
        P^\text{load,curt}_{n,k}:=P^\text{load,des}_{n,k}-P^\text{load}_{n,k}\,.
    \end{align}
\end{itemize}
\begin{remark}
Additional constraints can also be included in the formulation. For example, constraining the power factor could be important to alleviate power quality concerns. As such, we can place constraints such as:
\begin{align*}
    \left|Q_{n,k}^\text{pv}\right|\leq \gamma^*\left|P_{n,k}^\text{pv}\right|\, ~\text{and}~ \left|Q_{n,k}^\text{es}\right|\leq \gamma^*\left|P_{n,k}^\text{es}\right|\,, 
\end{align*}
where $\gamma^*>0$ is some suitably chosen values.
\end{remark}

The objective function of the optimization problem consists of costs of generating from the DG unit, and penalties on the solar and load curtailment. In this paper, we adopt a multi-period linear cost function defined as follows:
\begin{align}
    f(u):=\sum_k \sum_n \left(c_1 P^\text{dg}_{n,k}+c_2 P^\text{pv,curt}_{n,k}+c_3 P^\text{load,curt}_{n,k}\right)
\end{align}
where the parameters $c_{1,2,3}$ are chosen appropriately to reflect the cost (or, penalty) on each term. Several works in the literature, such as~\cite{parisio2014model,zhang2013robust}, have shown that using a linear cost function in microgrids is a reasonable assumption. The baseline optimization is then given as below:
\begin{align}\label{eq:baseline}
    \textsc{(baseline)}\qquad\min~f(u)\,,~\text{s.t.}~ \text{constraints \eqref{eq:pf_linear}-\eqref{eq:load_curt2}.}
\end{align}
%

==> ACC_sections/conclusions.tex <==
This paper presented a method to determine the adversarial set of a three-phase microgrid system. We formulate the robust optimization problem and from that we formulate the adversarial set characterization problem. We illustrate the inner approximation of the adversarial set through simulation results on IEEE-123 node distribution system. Future work will develop methods to incorporate the determined adversarial sets in microgrid planning and operation. Future work will also focus on probabilistic uncertainties (in the form of chance-constrained and risk based optimization), and compare the conservativeness of the characterized adversarial set between the deterministic and probabilistic approaches. Moreover, we will also investigate the applicability of this approach to larger systems (e.g., networked microgrids).

==> ACC_sections/intro.tex <==
\textit{Decarbonization}, \textit{digitalization}, and \textit{decentralization} are driving the evolution of the energy infrastructures worldwide in the 21st century \cite{di2018decarbonization}. There are incentives towards low carbon solutions (including, but not limited to, renewable energy resources), most of which are located at the customer sites (e.g., rooftop solar panels). On the other hand, advanced sensing and control technologies, coupled with ubiquitous communication infrastructure, are creating a digital platform for efficient and optimal utilization of distributed energy resources. Fueled by these and other drivers, microgrids are fast emerging as viable energy infrastructure. Microgrids are a group of flexible energy resources operating together locally as a single controllable entity, satisfying certain reliability, power quality, and adequacy standards \cite{farrokhabadi2019microgrid}. 
% 
% \subsubsection*{\textbf{Microgrid resiliency optimization}}
Safe and reliable operation of microgrids via optimal coordination of the flexible energy resources has drawn much attention in recent works \cite{parhizi2015state}. 
% 
% Algorithmic procedures are needed to ensure that such systems are designed to be resilient to a wide range of cyber-physical adversarial events. 
% % With increased disturbances and threats from adversarial attacks on cyber-physical systems, it becomes important to study the level of resiliency that can be provided by these systems in the face of contingencies. 
% This paper provides a robust optimization framework to quantify the largest adversarial perturbation that a system can accommodate without violating pre-specified resiliency metrics. We formulate the maximal adversarial set characterization as a bi-level optimization problem which is solved via Lagrangian relaxations. We illustrate the proposed algorithm on an islanded microgrid example: a modified IEEE 123-node feeder with distributed energy resources. Simulations are carried out to characterize the tolerable adversarial perturbations for varying levels of available flexibility (energy reserves).
% 
Several works, including~\cite{anderson2017increasing}, have shown how microgrids with multiple energy sources can minimize the cost of energy and increase the resilience of energy supply to critical loads. %
%Many such resiliency metrics have been developed in the literature which depend on the attributes of the specific microgrid and its location~\cite{mishra2021microgrid}. 
% Recent works such as~\cite{bajpai2016novel} have also considered extreme events when developing such resiliency metrics. 
In~\cite{hussain2019impact}, data-driven methods have been used to study the impact of uncertainties in the renewable generation on microgrid resiliency, whereas in~\cite{wu2019microgrid}, resiliency metrics are incorporated into the microgrid planning problem. A robust optimization framework for microgrid operation is presented in~\cite{liu2017robust}, which calculates the reserves required to ensure robustness under modeled uncertainties. 

% \subsubsection*{\textbf{Adversarial events characterization}} 
The resiliency of energy systems, e.g., microgrids, against various cyber and physical adversarial events, including malicious attacks, have been studied in the literature \cite{dehghani2021cyber,wang2019deep,dehghani2021blockchain,sahoo2018stealth}. One type of such attacks includes injecting measurement errors to renewable generation output. Such errors can be constant offsets or potentially time-varying, and left untreated, may eventually lead to ramp-induced attacks \cite{che2019impact}. Another class of attacks include \textit{replay attacks} \cite{habibi2020detection}, whereby the measured renewable generation output is maliciously changed to reflect the true generation at a previous time stamp, thus impacting dispatch decisions. A third class of attacks entails corruption of state estimation, whereby the estimated physical quantities required for dispatch decisions (such as load setpoints) are maliciously changed \cite{kushal2018risk,banerjee2021online}. Specifically, load-setpoint change attacks often cause maximal impact when affected during specific hours of the day (for example, during 12\,-\,7\,PM, when the load typically rises to hit an evening peak). A final class of attacks is coordinated attacks, whereby an attacker often has access to multiple critical information of the system, and can maliciously pose threats in a coordinated manner, from multiple sources (such as malicious under-estimation of load coupled with over-estimation of renewable capacity). Examples of such cyber-physical attacks can be found in~\cite{sun2018cyber,he2021tri,che2019impact}. 
% 
In addition to attacks, other physical events such as generator outage, loss of solar generation due to cloud coverage, etc., could also lead to violations of critical operational constraints (such as serviceability of critical loads), as considered in this work.

The main contribution of the paper is to identify the set of cyber-physical adversarial events that the microgrid is guaranteed to be resilient against, via optimal use of available flexible energy resources. An optimization problem is set up to construct an inner approximation of the tolerable adversarial set.
% 
The rest of the paper is organized as follows. Sec.\,\ref{sec:baseline} presents the microgrid model that will be used in this paper and presents baseline optimization results without considering the uncertainty due to adversarial events. Sec.\,\ref{sec:verification} provides the robust version of the microgrid optimization problem that calculates optimal reserves required to manage the adversarial events. Sec.\,\ref{sec:adv_set} provides the adversarial set characterization technique that is used to determine an inner approximation of the set of adversarial events that the microgrid can handle. Simulation results showing various case studies on the baseline model, robust model and adversarial set characterization are shown in Sec.\,\ref{sec:results}. Finally, Sec.\,\ref{sec:concl} provides the conclusions and the scope for future work.

==> ACC_sections/robust_optimization.tex <==
% Following an approach similar to \cite{liu2017robust}, 
We adapt the optimization problem \eqref{eq:baseline} to robustify it against a specified set of adversarial events. The main idea behind robustifying the optimization dispatch is to ensure \textit{sufficient reserves} in the dispatched resources (DG, PV, storage, and interruptible load) so that these can adjust their output in response to adversarial events. While we omit the detailed description of the robust formulation due to space limitations, and refer the interested readers to \cite{liu2017robust} (and the references therein), we present here the essential deviations from the baseline formulation \eqref{eq:baseline}.
% 
The adversarial events are grouped into the \textit{event} (or, perturbation) vector $w$\,, which may represent various cyber-physical attacks and/or physical disruptions. For example, an outage in DG could be represented by an uncertainty in the parameter $\overline{S}^\text{dg}_{n,k}$\,. Likewise, a load-masking attack could be represented by an uncertainty in $P^\text{load,des}_{n,k}$\,, while a sudden loss in solar generation could be represented by an uncertainty in $\widehat{P}^\text{pv}_{n,k}$\,. In this paper, we consider a bounded set of uncertainties:
\begin{align}
    w\in\Omega_W\,.
\end{align}
% 
In the most general form, the robust optimization problem for a system can be expressed in the following form:
\begin{subequations}\label{eq:arbit_opt}
   \begin{align}
   & \min_{u} \max_{{w}} f({u},w)\\
    s.t. & \ g({u},{w}) \le 0 \qquad \forall {w}\in \Omega_W
\end{align}
\end{subequations}
where $g({u},{w})$ are the constraints \eqref{eq:pf_linear}-\eqref{eq:load_curt2}. The above optimization problem \eqref{eq:arbit_opt} can be converted to a robust formulation using the \textit{explicit maximization method} (see \cite{bai2015robust}) in the following form:
\begin{align}
       \min_{{u}} \widehat{f}({u})\,,\quad \text{s.t.} \,~\widehat{g}({u}) \le 0 
\end{align}
where $\widehat{f}({u})\!=\!\max_{{w}} f({u},{w})$ and $\widehat{g}({u})\!=\!\max_{{w}} g({u},{w})$. The new model does not contain any disturbance terms and if the functions $\widehat{f}({u})$ and $\widehat{g}({u})$ are convex, then the optimization problem is convex, which can be solved efficiently. 


The additional decision variables we consider in our robust formulation include:
\begin{itemize}
    \item \textit{Solar reserves}: These are the up ($R^{\text{pv}+}_{n,k}>0$) and down ($R^{\text{pv}-}_{n,k}>0$) reserves set aside on the solar generation dispatch, so that the solar output has flexibility to increase or decrease from the optimally dispatched amount ($P^\text{pv}_{n,k}$) in response to an adversarial event:
    \begin{align}
        R^{\text{pv}-}_{n,k}\leq {P}^\text{pv}_{n,k}\leq \widehat{P}^\text{pv}_{n,k}-R^{\text{pv}+}_{n,k}
        \label{eq:pv_reserves}
    \end{align}
    
    \item \textit{DG reserves}: These are the up ($R^{\text{dg}+}_{n,k}>0$) and down ($R^{\text{dg}-}_{n,k}>0$) reserves set aside on the DG dispatch:
    \begin{align}
        R^{\text{dg}-}_{n,k}\leq {P}^\text{dg}_{n,k}\leq \overline{S}^\text{dg}_{n,k}-R^{\text{dg}+}_{n,k}
        \label{eq:dg_reserves}
    \end{align}
    
    \item \textit{Storage reserves}: These are the up ($R^{\text{es}+}_{n,k}>0$) and down ($R^{\text{es}-}_{n,k}>0$) reserves set aside on the storage dispatch, allocated in such a way that there is flexibility on both the charging/discharging rates, as well as the SoC limits (assuming a look-ahead period of $\Delta t$):
    \begin{subequations}
           \begin{align}
    -\overline{P}^\text{es}_{n,k}+R^{\text{es}-}_{n,k}&\leq {P}^\text{es}_{n,k}\leq \overline{P}^\text{es}_{n,k}-R^{\text{es}+}_{n,k}\\
    \underline{E}_n^\text{es} + R^{\text{es}+}_{n,k}\Delta t&\leq E_{n,k}^\text{es}\leq \overline{E}_n^\text{es}-R^{\text{es}-}_{n,k}\Delta t\,.
    \end{align}
     \label{eq:es_reserves}
    \end{subequations}
    
    \item \textit{Load reserves}: These are the up ($R^{\text{load}+}_{n,k}>0$) and down ($R^{\text{load}-}_{n,k}>0$) reserves set aside on the load dispatch (note the reverse convention on direction):
    \begin{align}
    P^\text{load,min}_{n,k}+R^{\text{load}+}_{n,k}\leq P^\text{load}_{n,k}\leq P^\text{load,des}_{n,k}-R^{\text{load}-}_{n,k}
        \label{eq:load_reserves}
    \end{align}
\end{itemize}





The goal of the robust microgrid optimization is then to minimize the cost of dispatched generation and reserves while satisfying the device and network constraints for all the disturbances in the selected disturbance set $\Omega_w$. Combining the additional reserves cost and the additional constraints \eqref{eq:pv_reserves}-\eqref{eq:load_reserves}, we develop the following robust formulation:
\begin{subequations}
\label{eq:robust}
       \begin{align}
       \textsc{(robust)}\,~\, \min_{{u}} & \,~\widehat{f}({u})+f^\text{R}(\textbf{R}^{\text{pv}}_{n,k},\textbf{R}^{\text{dg}}_{n,k},\textbf{R}^{\text{es}}_{n,k},\textbf{R}^{\text{load}}_{n,k})\\
       \text{s.t.} \,~&\,~\widehat{g}({u}) \le 0\,,\,~\text{constraints \eqref{eq:pv_reserves}-\eqref{eq:load_reserves}} 
\end{align}
\end{subequations}
where the bold-faced $\textbf{R}^{\text{pv}}_{n,k}=(R^{\text{pv}+}_{n,k},\,R^{\text{pv}-}_{n,k})$ and likewise, while $f^R$ is a linear cost function of the allocated reserves, defined similarly as $f$\,. 

Finally, we implement a simple measurement based control algorithm that dispatches reserves in response to disturbance events. In microgrids, the amount of flexible generation is increased/decreased based on real-time frequency measurements. In our quasi-static analysis, we consider the supply-demand power imbalance to be the measure of frequency and utilize that to dispatch the microgrid reserves in order to meet the demand under disturbance events. While works such as \cite{brahma2020optimal} has explored such feedback control methods, in this work, we employ a simple proportional controller that dispatches reserves in proportion to their available capacity:
\begin{align*}
    Reserve \  Dispatch=\frac{Reserve \  Capacity}{Total \  Reserves}*Imbalance\,.
\end{align*}
%
% In future analysis we will develop more thorough and sophisticated control algorithms .

% \subsection{Main Problem} 









==> ACC_sections/scenarios.tex <==
The resiliency of energy systems (including microrgids) against various cyber and physical adversarial events, including malicious attacks, have been studied in the literature \cite{dehghani2021cyber,wang2019deep,dehghani2021blockchain,sahoo2018stealth}. One type of such attack includes injecting measurement errors to renewable generation output. Such errors can be constant offsets or potentially time-varying, and left untreated, may eventually lead to ramp-induced attacks \cite{che2019impact}. Another class of attacks include \textit{replay attacks} \cite{habibi2020detection}, whereby the measured renewable generation output is maliciously changed to reflect the true generation at a previous time stamp, thus impacting dispatch decisions. A third class of attacks entails corruption of state estimation, whereby the estimated physical quantities required for dispatch decisions (such as load setpoints) are maliciously changed \cite{kushal2018risk}, \cite{banerjee2021online}. Specifically, load-setpoint change attacks often cause maximal impact when affected during specific hours of the day (for example, during 12pm - 7pm, when load typically rises to hit an evening peak). A final class of attacks is coordinated attacks, whereby an attacker often has access to multiple critical information of the system, and can maliciously pose threats in a coordinated manner, from multiple sources (such as malicious under-estimation of load coupled with over-estimation of renewable capacity). Examples of such attacks, which often include attacks in both the cyber as well as the physical layer can be found in~\cite{sun2018cyber}, \cite{he2021tri}, \cite{che2019impact}. 
% 
In addition to malicious attacks, other physical events such as generator outage, loss of solar generation due to cloud coverage, etc., could also lead to violations of critical operational constraints (such as serviceability of critical loads) as specified in Sec.\,\ref{sec:baseline}. In the following, we describe a robust extension of \eqref{eq:baseline}.



% These can be broadly grouped into the following categories, as shown below:

% \begin{itemize}
%     \item \textbf{Injecting measurement errors into PV generation output:} Within this type of attack, we can have several possibilities:
%     \begin{itemize}
%         \item Inject $\epsilon$ error to the PV generation at all time stamps, i.e.,
%         $$\hat{S}_{n,k}^S = S_{n,k}^S\times (1+\epsilon),$$ where $\epsilon \in [-1,1]$. The factor $\epsilon$ can be tweaked to emulated systematic under-estimations as well as over-estimations.
%         %For implementation purpose, we can treat $\epsilon$ to be a parameter, and vary in discrete steps, such as $\epsilon = \{0.1, 0.2, 0.3\}$. 
%         \item Inject time-varying errors instead of static error.
%     \end{itemize}
%     These type of error, left untreated, can lead to ramp-induced attacks (RID), as discussed in details in \cite{che2019impact}.
    
%     \item \textbf{Injecting latency to PV generation output measurement (Replay attack):} In this type of attack (see, for example \cite{habibi2020detection}), the measured PV-generation output is maliciously changed to reflect the true generation at a previous time stamp (with $\delta$ delay). Mathematically, $$\hat{S}_{n,k}^S = S_{n,k-\delta}^S,$$ where $\hat{S}^S$ denotes the measured PV-generation output to be used in the microgrid optimization.
    
%     \item \textbf{Injecting errors to load measurement (corrupted state estimation):} This type of attack is also known as load curtailment cyber-attack (see \cite{kushal2018risk}, \cite{banerjee2021online} for detailed case studies). Similar to generation setpoint change attack, assuming $\epsilon$ to be the malicious error injection, we can write:
%     $$ \hat{S}_{n,k}^L = S_{n,k}^L \times (1 + \epsilon), $$
%     Note that as given in \cite{kushal2018risk}, it may be optimal for the attacker (causing maximal disruption) when this type of attack is initiated around afternoon (12 pm) and continued till peak evening hours. 
    
%     \item \textbf{Partial/complete loss of dispatchable generation capability}
    
%     \item \textbf{Coordinated attack schemes:} In this type of attack, the attacker often has access to multiple critical information of the system, and is in a position to maliciously pose threats in a coordinated manner, from multiple sources. Examples of such attacks, which often include attacks in both the cyber as well as the physical layer can be found in~\cite{sun2018cyber}, \cite{he2021tri}, \cite{che2019impact}.
%     %In our work, we consider at least 1 type of coordinated attack scheme, where the attacker can simultaneously inject error signals to load estimation as well as PV-forecast, such that load is under-estimated and PV-generation is over-estimated, so that the real time generation-load imbalance is magnified, thus upsetting real time grid operations.
% \end{itemize}

==> report_chapters/Appendices.tex <==
\appendix

\section{appendix section 1}

\subsection{subsection title}


\paragraph{paragraph title}


\section{appendix section 2}

==> report_chapters/Conclusions.tex <==
\section{Conclusions}

==> report_chapters/Introduction.tex <==
\section{Introduction}

\stitle{Background} 

\stitle{Objectives} 


\subsection{Technical Approach and Accomplishments}



\stitle{Accomplishments} 

\subsection{Report Structure}
The rest of this technical report is organized as follows. 

==> report_chapters/acronyms.tex <==
\acronyms
\begin{acrolist}
\item{}{}   % use this blank item entry for better alignment of the rest
\item{ALERT}{Adaptive Learning-Enabled Resilient Tuning}
\item{PNNL}{Pacific Northwest National Laboratory}
\end{acrolist}

==> report_chapters/musings.tex <==
\section{Virtual Whiteboard}

\subsection{Microgrid Economic Objectives}
Key questions:
\begin{itemize}
    \item What kind of resources are available? What are the corresponding decision variables? What simplifying assumptions are made?
    \item What is the microgrid operator's economic objective?
    \item What kind of power flow equations should be considered? (The feeder model is 3 phase unbalanced)
    \item How should the electrical boundary between the microgrid and the rest of the feeder be considered?
\end{itemize}

\subsection{Optimization Problem for Slides}

\begin{align}
 \min \sum_k\sum_n& \left[c_1(P^{\text{b}}_{n,k})+c_2(P^{\text{G}}_{n,k})\right.\notag\\
 &+c_3(P^{\text{Sc}}_{n,k})+c_4(P^{\text{Lc}}_{n,k})\notag\\
 &\left.+\widetilde{c}_1(\Delta P^{\text{b}}_{n,k})+\widetilde{c}_2 (\Delta P^{\text{G}}_{n,k})\right]\label{eq:P2_obj}\\
 \\
\text{s.\,t.\,,}~\forall (l,n,\textbf{w})&\in\calL\times\calN\times\Omega_w:\notag\\
\\
0&=\mathbf{F}(S^b_{n,k},S^G_{n,k},S^S_{n,k},S^L_{n,k})\notag\\
0&\leq S_{\text{max},l}(\textbf{w}) - \left|\text{diag}(S_{l,k})\right|&\forall l\in \mathcal{L}\notag\\
V_{\text{min},n}^2&\leq \text{diag}(W_{n,k})\leq V_{\text{max},n}^2 &\forall n\in \mathcal{N}\notag\\
\\
0&\leq G_{\text{max},n}(\textbf{w}) - \left|S^{\text{S}}_{n,k}+\Delta S^{\text{S}}_{n,k}\right|&\forall n\in \mathcal{N}\notag\\
0&\leq D_{\text{max},n}(\textbf{w})- \left|S^{\text{G}}_{n,k}+\Delta S^{\text{G}}_{n,k}\right| &\forall n\in \mathcal{N}\notag\\
0&\leq H_{\text{max},n}(\textbf{w})-\left|S^{\text{b}}_{n,k}+\Delta S^{\text{b}}_{n,k}\right| &\forall n\in \mathcal{N}\notag\\
\\
0&=E_{n,k+1}-E_{n,k}+\eta_{\text{b},n}P^{\text{b}}_{n,k}\Delta t &\forall n\in \mathcal{N}\notag\\
P^{\text{b}}_{n,k}&\in\left[\Delta P^{\text{b}}_{n,k}\,,\, P_{\text{max},n}(\textbf{w})-\Delta P^\text{b}_{n,k}\right] &\forall n\in \mathcal{N}\\
E_{n,k}&\in \left[E_{\text{min},n}(\textbf{w})+\Delta E_{n,k}\,,\, E_{\text{max},n}(\textbf{w})-\Delta E_{n,k}\right] &\forall n\in \mathcal{N}\notag
\end{align}

==> report_chapters/task1_baseline.tex <==
\section{Task 1 Single Microgrid Baseline Control}\label{S:task1_baseline}

The goal of this task is to identify and implement the baseline controls for the single microgrid use-case. In particular, we will leverage the co-simulation framework (FNCS, GridLAB-D, Julia/Python) developed at PNNL under ENERGISE project to implement an optimal dispatch problem as the baseline for a single microgrid with high renewable penetration (at least 50\%). The baseline optimal dispatch controller would be sending active and reactive power set-points to various DERs (e.g., solar inverters, battery storage, flexible loads), based on various sensor measurements and forecasts.

\subsection{Nomenclature}

\begin{table}[ht!]
\begin{tabular}{ll}
\textbf{Symbol}                             & \textbf{Meaning}                                                       \\
$\mathcal{N}$                      & Set of nodes in the microgrid                                 \\
$\mathcal{N}_m$                      & Set of neighboring nodes for node $m$ in the microgrid                                 \\
$\mathcal{E}$                      & Set of edges (lines) in the microgrid                         \\
$\mathcal{S_C}$                      & Set of nodes containing DG units                              \\
$\mathcal{S_R}$                      & Set of nodes containing renewable DERs (PV inverter nodes)                                 \\
$\mathcal{P}_n$                    & Set of phases at node $n$                                     \\
$\mathcal{P}_{mn}$                 & Set of phases of line $(m,n)$                                 \\
$V_{n}^{\phi}$                     & Complex line-to-neutral voltage at phase $\phi$ of node $n$   \\
$I_{n}^{\phi}$                     & Complex current injected at phase $\phi$ of node $n$          \\
$I_{m\rightarrow n}^{\phi}$        & Complex current on phase $\phi$ of line $(m,n)$               \\
$P_{i,n}^{\phi} (Q_{i,n}^{\phi})$  & Net active (reactive) power injection at phase $\phi$ of node $n$     \\
$P_{L,n}^{\phi} (Q_{L,n}^{\phi})$  & Active (reactive) load demand at phase $\phi$ of node $n$     \\
$P_{r,n}^{\phi}$  & Uncontrollable active (reactive) generation at phase $\phi$ of node $n$     \\
$P_{c,n}^{\phi}$  & Active (reactive) load curtailed at phase $\phi$ of node $n$     \\
$P_{b,n}^{\phi}$  & Battery power injected at phase $\phi$ of node $n$     \\
$P_{G,n}^{\phi} (Q_{G,n}^{\phi})$  & Active (reactive) power generated at phase $\phi$ of node $n$ \\
$y_{C,n}$                          & Susceptance of a capacitor at phase $\phi$ of node $n$        \\
$P_{m\rightarrow n}$               & Active power exiting node $n$ of line $(m,n)$                 \\
$\mathbf{Z}_{mn}$                  & Phase impedance matrix of line $(m,n)$                        \\
$\mathbf{Y}^{(s)}_{mn}$            & Shunt admittance matrix of line $(m,n)$                       \\
$V_n^{\min},\ V_n^{\max}$          & Allowable bounds for voltage magnitude at node $n$            \\
$P_{G,n}^{\min}\ (Q_{G,n}^{\min})$ & Minimum active (reactive) power generated at node $n$         \\
$P_{G,n}^{\max}\ (Q_{G,n}^{\max})$ & Maximum active (reactive) power generated at node $n$         \\
                                   &                                                               \\
                                   &                                                              
\end{tabular}
\end{table}


\subsection{Optimization Formulation}

\noindent Consider a look-ahead horizon $\mathcal{K} = \{1,2,3,\ldots,K\}$. Assume that node $0$ is the reference node, where we hold $V_n^{\phi}|_{n = 0},\ \forall \phi \in \mathcal{P}_0$, as constants, i.e., phasor reference. Also, given a vector $\mathbf{v}$ and a matrix $\mathbf{V}$, let $[\mathbf{v}]_{\mathcal{P}}$ denote a $|\mathcal{P}|\times 1$ sub-vector containing entries of $\mathbf{v}$ indexed by $\mathcal{P}$. Also, denote $[\mathbf{V}]_{\mathcal{P}_1,\mathcal{P}_2} $ as the $|\mathcal{P}_1| \times |\mathcal{P}_2|$ sub-matrix with row and column indexed by $\mathcal{P}_1$ and $\mathcal{P}_2$ respectively. Define the optimization decision variable vector as follows:
\begin{equation}
    \mathbf{x} = \{ I_{0,k}^{\phi}\ \forall \phi \in \mathcal{P}_0, V_{n,k}^{\phi}, I_{n,k}^{\phi}, P_{G,n,k}^{\phi}, Q_{G,n,k}^{\phi}, \forall \phi \in \mathcal{P}_n,\ \forall n \in \mathcal{N}\setminus\{0\},\ \forall k \in \mathcal{K}\}.
\end{equation}
\textbf{Goal:} Given the demand $\{P_{L,n,k}^{\phi},Q_{L,n,k}^{\phi}\}$, find voltages ($V_{n,k}^{\phi}$), currents ($I_{n,k}^{\phi}$), and generation setpoints from DG units ($P_{G,n,k}^{\phi},Q_{G,n,k}^{\phi}$) so that steady state operation of the microgrid is optimal. The following cost functions ($J$) can be selected \cite{dall2013distributed}:
\begin{enumerate}
    \item \textbf{Network loss minimization plus penalize load curtailment:} \\ $J = \displaystyle\sum_{k=1}^K\displaystyle\sum_{(m,n)\in\mathcal{E}}\Big( P_{m\rightarrow n,k} + P_{n \rightarrow m,k}\Big) + \displaystyle\sum_{k=1}^K \displaystyle\sum_{n\in \mathcal{N}\setminus \mathcal{S}} \lambda_{pen,n} \displaystyle\sum_{\phi \in \mathcal{P}_n} P_{c,n,k}^{\phi}$,\\ where  $P_{m \rightarrow n,k} = \displaystyle\sum_{\phi \in \mathcal{P}_{mn}}V_{m,k}^{\phi} (I_{m\rightarrow n,k}^{\phi})^*$.
    
    \item \textbf{Generation cost minimization plus penalize load curtailment:}\\ $J =  \displaystyle\sum_{k=1}^Kc_{0,k}\displaystyle\sum_{\phi\in \mathcal{P}_0} V_{0,k}^{\phi}(I_{0,k}^{\phi})^* + \displaystyle\sum_{k=1}^K\displaystyle\sum_{s\in\mathcal{S}}c_s\displaystyle\sum_{\phi \in \mathcal{P}_s}P_{G,s,k}^{\phi} + \displaystyle\sum_{k=1}^K \displaystyle\sum_{n\in \mathcal{N}\setminus \mathcal{S}} \lambda_{pen,n} \displaystyle\sum_{\phi \in \mathcal{P}_n} P_{c,n,k}^{\phi}$.\\ 
    \newline
    Note that costs of procuring power from the slack node (alternatively referred to as the point of contact/PCC) and the DG unit $s$, are $c_0>0$, and $c_s \geq 0$, respectively. Also, note that the first objective is equivalent to the second when $c_{0,k} (\forall k) = c_s = 1$.
\end{enumerate}

\textbf{Constraints:} 
\begin{eqnarray}
V_{s,k}^{\phi}(I_{s,k}^{\phi})^* & = & P_{G,s,k}^{\phi} - P_{L,s,k}^{\phi} + j(Q_{G,s,k}^{\phi} - Q_{L,s,k}^{\phi}),\ \forall \phi \in \mathcal{P}_s,\ s \in \mathcal{S_C},\ \forall k \in \mathcal{K},\\
V_{n,k}^{\phi}(I_{n,k}^{\phi})^* &=& P_{i,n,k}^{\phi} + jQ_{i,n,k}^{\phi} + jy_{C,n}^{\phi}|V_{n,k}^{\phi}|^2,\ \forall \phi \in \mathcal{P}_n,\ n \in \mathcal{N}\setminus \mathcal{S_C},\ \forall k \in \mathcal{K},\\
P_{i,n,k}^{\phi} &=& P_{r,n,k}^{\phi} + P_{b,n,k}^{\phi} - P_{L,n,k}^{\phi} + P_{c,n,k}^{\phi},\forall \phi \in \mathcal{P}_n,\ \ n \in \mathcal{N}\setminus \mathcal{S_C},\ \forall k \in \mathcal{K},\\
Q_{i,n,k}^{\phi} &=& Q_{r,n,k}^{\phi} + Q_{b,n,k}^{\phi} - Q_{L,n,k}^{\phi},\ \forall \phi \in \mathcal{P}_n,\ \ n \in \mathcal{N}\setminus \mathcal{S_C},\ \forall k \in \mathcal{K},\\
E_{b,n,k+1}^{\phi} &=& E_{b,n,k}^{\phi} + \eta P_{b,n,k}^{\phi},\ \forall \phi \in \mathcal{P}_n\ , n \in \mathcal{N}\setminus \mathcal{S_C},\ \forall k \in \mathcal{K},\\
E_{b}^{-} & \leq& E_{b,n,k}^{\phi} \leq E_b^{+},\ n \in \mathcal{N}\setminus \mathcal{S_C},\ \forall \phi \in \mathcal{P}_n,\ \forall k \in \mathcal{K},\\
E_{b,n,k}^{\phi}|_{k=0} &=& E_{b,n,0}, \ \forall \phi \in \mathcal{P}_n,\ \forall k \in \mathcal{K},\\
P_{b,n}^{-} &\leq& P_{b,n,k}^{\phi} \leq P_{b,n}^{+},\ n \in \mathcal{N}\setminus \mathcal{S_C},\ \forall \phi \in \mathcal{P}_n,\ \forall k \in \mathcal{K},\\
I_{n,k}^{\phi} &=&  \displaystyle\sum_{m\in\mathcal{N}_n} \Big[\Big(\frac{1}{2}\mathbf{Y}_{mn}^{(s)} + \mathbf{Z}_{mn}^{-1}\Big)[\mathbf{v}_{n,k}]_{\mathcal{P}_{mn}} - \mathbf{Z}_{mn}^{-1} [\mathbf{v}_{m,k}]_{\mathcal{P}_{mn}}\Big]_{\{\phi\}},\ \forall \phi \in \mathcal{P}_n, n \in \mathcal{N},\forall k \in \mathcal{K},\\ 
V_n^{\min} &\leq& |V_{n,k}^{\phi}| \leq V_n^{\max},\ \forall \phi \in \mathcal{P}_n,\ n \in \mathcal{N},\ \forall k \in \mathcal{K},\\
P_{G,s}^{\min} &\leq& P_{G,s,k} \leq P_{G,s}^{\max},\ \forall \phi \in \mathcal{P}_s, s \in \mathcal{S_C},\ \forall k \in \mathcal{K},\\
Q_{G,s}^{\min} &\leq& Q_{G,s,k} \leq Q_{G,s}^{\max},\ \forall \phi \in \mathcal{P}_s, s \in \mathcal{S_C},\ \forall k \in \mathcal{K},\\
\Delta P_{G,s}^{-} &\leq& P_{G,s,k}^{\phi} - P_{G,s,k-1} \leq \Delta P_{G,s}^{+},\ \forall \phi \in \mathcal{P}_s, \forall s \in \mathcal{S_C},\ \forall k \in \mathcal{K}\setminus\{1\},\\
P_{r,s}^{\min} &\leq& P_{r,s,k} \leq P_{r,s}^{\max},\ \forall \phi \in \mathcal{P}_s, s \in \mathcal{S_R},\ \forall k \in \mathcal{K},\\
Q_{r,s}^{\min} &\leq& Q_{r,s,k} \leq Q_{r,s}^{\max},\ \forall \phi \in \mathcal{P}_s, s \in \mathcal{S_R},\ \forall k \in \mathcal{K},\\
(P_{r,n,k}^{\phi})^2 + (Q_{r,n,k}^{\phi})^2 &\leq& S_{r,n,rated}^2,\ \forall \phi \in \mathcal{P}_n,\ \forall n \in \mathcal{S_R},\ \forall k \in \mathcal{K},\\
P_{r,n,k}^{\phi} &=& Q_{r,n,k}^{\phi} = 0,\ \forall \phi \in \mathcal{P}_n,\ \forall n \in \mathcal{N} \setminus (\mathcal{S_C}\cup \mathcal{S_R}),\\
0 &\leq& P_{c,n,k}^{\phi} \leq P_{c,n,k}^{\max},\ \forall \phi \in \mathcal{P}_n,\ \forall n \in \mathcal{N}\setminus \mathcal{S_C},\ \forall k \in \mathcal{K}. 
\end{eqnarray}

\noindent The aforementioned problem is a non-convex, nonlinear program and needs adaptation to more suitable relaxed forms for easier implementation.

The optimization problem can also be expressed in the Branch Flow Model (BFM) formulation as shown below. For the branch flow formulation we introduce the following notation:\\
Let $V_{n,k}$ denote the $|\mathcal{P}|\times 1$ sub-vector containing entries of $V_{n,k}^{\phi}$, $i_{l,k}$ denote the $|\mathcal{P}|\times 1$ sub-vector containing entries of $I_{m\rightarrow n}^{\phi}$, where $\mathcal{L}=\{1, 2, . . . , l\}= \{(m,n)\}\subset (\mathcal{N}\times \mathcal{N})$ is the set of all branches. Let $S_{l,k}$ denote the $|\mathcal{P}|\times 1$ sub-vector containing entries of $P_{m \rightarrow n}$, $Z_l$ be the impedance matrix of line $l$, $S_{n,k}^{\text{net}}$ be the net complex power injection, $S^{\text{S}}_{n,k}$ be the complex solar power generation, $S^{\text{L}}_{n,k}$ be the complex load and $S^{\text{b}}_{n,k}=P^{\text{b}}_{n,k}+i q^{\text{b}}_{n,k}$ be the complex battery power injection. Let $E_{n,k}$ be the battery state of charge and $\eta_{\text{b},n}$ be the battery efficiency. Also let $S^{\text{G}}_{n,k}$ be the complex power from the diesel generator and let $P^{\text{Lc}}_{n,k}$ be the load curtailment and 
$P^{\text{Sc}}_{n,k}$ be the solar curtailment. Then the constraints can be formulated in the Branch Flow Model (BFM) as:
\begin{align}
% &\min_{P^{\text{b}}_{n,t},q^{\text{b}}_{n,t},S^{\text{S}}_{n,t}}f(x)\label{eq:P1_obj}\\
&\begin{bmatrix}
W_{n,k} & S_{l,k}\\
S_{l,k}^{*} & I_{l,k}\end{bmatrix}=
\begin{bmatrix}
V_{n,k}\\
i_{l,k}\end{bmatrix}
\begin{bmatrix}
V_{n,k}\\
i_{l,k}\end{bmatrix}^{*} \qquad \forall l\in \mathcal{L}\label{eq:P1_BFM}\\
0=&W_{n,k}-W_{m,k}+(S_{l,k}Z_l^*+Z_lS_{l,k})-Z_lI_{l,k}Z_l^*\ \ \forall l\in \mathcal{L}\label{eq:P1_volt_rel}\\
0=&\text{diag}(S_{l,k}-Z_l I_{l,k}-\sum_{p}S_{p,k})+S^{\text{net}}_{n,k}\ \ \ \forall l\in \mathcal{L}\label{eq:P1_power_balance}\\
0=&\text{real}(S^{\text{net}}_{n,k}-S^{\text{S}}_{n,k}-S^{\text{G}}_{n,k}-S^{\text{b}}_{n,k}+S^{\text{L}}_{n,k})+P^{\text{Sc}}_{n,k}-P^{\text{Lc}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P1_node_real_balance}\\
0=&\text{imag}(S^{\text{net}}_{n,k}-S^{\text{S}}_{n,k}-S^{\text{G}}_{n,k}-S^{\text{b}}_{n,k}+S^{\text{L}}_{n,k})-Q^{\text{Lc}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P1_node_reactive_balance}\\
&|\text{diag}(S_{l,k})|\leq S_{\text{max},l} \qquad \forall l\in \mathcal{L}\label{eq:P1_line_const}\\
&V_{\text{min},n}^2\leq \text{diag}(W_{n,k})\leq V_{\text{max},n}^2 \ \forall n\in \mathcal{N}\label{eq:P1_volt_const}\\
&(\text{real}(S^{\text{S}}_{n,k})-P^{\text{Sc}}_{n,k})^2+\text{imag}(S^{\text{S}}_{n,k})^2|\leq G_{\text{max},n}^2 \qquad \forall n\in \mathcal{N}\label{eq:P1_solar_inv_limit}\\
&|S^{\text{G}}_{n,k}|\leq D_{\text{max},n} \qquad \forall n\in \mathcal{N}\label{eq:P1_diesel_inv_limit}\\
&(P^{\text{b}}_{n,k})^2+(q^{\text{b}}_{n,k})^2\leq H_{\text{max},n}^2, \qquad \forall n\in \mathcal{N}\label{eq:P1_battery_inv_limit}\\
0=&E_{n,k+1}-E_{n,k}+\eta_{\text{b},n}P^{\text{b}}_{n,k}\Delta t \qquad \forall n\in \mathcal{N}\label{eq:P1_battery_power_rel}\\
&E_{\text{min},n}\leq E_{n,k}\leq E_{\text{max},n} \qquad \forall n\in \mathcal{N}\label{eq:P1_SOC_limit}\\
 0\leq & P^{\text{b}}_{n,k}\leq P_{\text{max},n} \qquad \forall n\in \mathcal{N}\label{eq:P1_Pd_limit}
\end{align}

The non-convexity in the above BFM is due to the non-linear constraint in~\eqref{eq:P1_BFM}. 
This constraints make the problem NP-hard. The nonlinear equality constraint in~\eqref{eq:P1_BFM} can equivalently be expressed by the following two constraints %~\cite{gan2014convex}:
 \begin{equation}\label{eq:SDP_relax}
\begin{bmatrix}
W_{n,k} & S_{l,k}\\
S_{l,k}^* & I_{l,k}\end{bmatrix} \succeq 0, \ \ \
rank\begin{bmatrix}W_{n,k} & S_{l,k}\\
S_{l,k}^* & I_{l,k}\end{bmatrix} = 1\\
\end{equation}
The inequality constraint in~\eqref{eq:SDP_relax} is a positive semi-definte (PSD) convex constraint, whereas the rank constraint is non-convex. Removing the rank constraint in~\eqref{eq:SDP_relax} leads to a convex SDP formulation, however, it is desirable to find a second order cone relaxation that can be solved with numerically robust solvers such as GUROBI. %~\cite{gurobi}.
SOCP relaxation can be applied to the PSD constraint in~\eqref{eq:SDP_relax} 
%as in~\cite{kocuk2016strong,horn2012matrix} 
to obtain the following relaxed SOC constraints:, 
\begin{align}\label{eq:SOC_relax1}
\left\lVert
\frac{2W_{n,k}(i,j)}
{W_{n,k}(i,i)-W_{n,k}(j,j)}\right\rVert
_2 & \leq W_{n,k}(i,i)+W_{n,k}(j,j)\\
%\end{equation}
%\begin{equation}
\label{eq:SOC_relax2}
\left\lVert
\frac{2I_{l,k}(i,j)}
{I_{l,k}(i,i)-I_{l,k}(j,j)}\right\rVert
_2 & \leq I_{l,k}(i,i)+I_{l,k}(j,j)\\
%\end{equation}
%\begin{equation}
\label{eq:SOC_relax3}
\left\lVert
\frac{2S_{l,k}(i,j)}
{W_{n,k}(i,i)-I_{l,k}(j,j)}\right\rVert
_2 & \leq W_{n,k}(i,i)+I_{l,k}(j,j)
\end{align}

The optimization model now becomes convex and can be solved with GUROBI (as a QCQP) or MOSEK (as an SOCP). 

However, the relaxation of the nonlinear power flow model in~\eqref{eq:P1_BFM}  with the second-order cone constraints~\eqref{eq:SOC_relax1}-\eqref{eq:SOC_relax3} can result in non-physical solutions to the OPF problem.% as has recently been shown in~\cite{wang2018chordal}.

Thus, if we seek a physically realizable solution for a general objective function, we need a nonlinear programming (NLP) formulation.  Thus, we seek to leverage the multi-period solution available from the SOCP. However, NLPs are not scalable and the solve time increases dramatically with the increase in problem size (and coupling).
%~\cite{boyd2004convex}
%\deleted{as can be seen from Fig.~\ref{fig:time_horizon_nlp}, which shows the increase in solve time as the length of the prediction horizon increases}.
To overcome this challenge, we propose a time-decoupled approach by fixing the battery's active power set-points in the NLP based on the solution obtained from the SOCP. This allows the NLP to focus on reactive power set-points and voltage limits. %, which aligns with recent analysis~\cite{molzahn2017computing}. In~\cite{molzahn2017computing}, it is shown how reactive power and voltage limits lead to disconnections in the power flow solution space resulting in a non-zero duality gap for the relaxed OPF.
Based on these observations, an SOCP-NLP coupled algorithm is developed  as shown in Fig.~\ref{fig:SOCP_NLP}, where the solution obtained from the SOCP is passed to the NLP solver. 
Prior work in literature %, such as~\cite{kocuk2016strong}, 
have proposed the idea of using the solution of a convex relaxation as an initial starting point for solving the full, nonlinear ACOPF. However, herein we extend the notion of a ``warm start'' to the multi-period domain. Specifically, we decouple the multi-period NLP by fixing the active power set-points of the batteries to the solution of the convex relaxation (SOCP).
Keeping the active power solutions constant leads to fixing the state of charge of the batteries and, as a result, results in a decoupling of the time-steps of the prediction horizon in the NLP. Thus, each time-step can be solved independently and in parallel (as independent NLPs), which  leads to a scalable implementation compared to solving the multi-period NLP.

\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{report_chapters/images/SOCP_NLP.png}
\caption{\label{fig:SOCP_NLP}Coupling of SOCP with NLP by fixing real power solutions from SOCP and hence decoupling the NLP to obtain a feasible solution.}
\end{figure}

This is further explained through Fig.~\ref{fig:SOCP_NLP_time} where for each time-step of the prediction, the reactive power range available to the NLP is constrained by the SOCP's solution. That is, Figure~\ref{fig:SOCP_NLP_time} illustrates the decomposition approach presented herein by showing the effect of the SOCP's optimized active power trajectory on the feasible set of the reactive power of the NLP problem.
\begin{figure}[h]
\centering
\includegraphics[width=0.39\textwidth]{report_chapters/images/Illus_fig_IL.png}
\caption{\label{fig:SOCP_NLP_time} Available reactive power variation range for NLP across multiple time steps based on the active power trajectory provided by the SOCP.}
\end{figure}
\begin{remark}

The decoupling of the time-steps reduces the feasible set of the optimization problem and, hence, increases the optimal value. Thus, the decoupled problem represents an upper bound on the time-coupled nonlinear problem, which in turn is lower bounded by the SOCP as shown below:
\begin{equation}\label{soc_nlp_relation}
    SOCP_{opt}\leq NLP_{opt}\leq DNLP_{opt}
\end{equation}
where $NLP_{opt}$ represents the optimal value of the time-coupled nonlinear program and $DNLP_{opt}$ the optimal value of the time-decoupled nonlinear program (DNLP).
\end{remark}
%Furthermore, the hot-start of the NLP with the solution of the SOCP leads to a faster convergence to a solution that is close to the global optimum, as compared to the flat start~\cite{castillo2013computational}-\cite{wu2001initialisation}.
The DNLP problem at each time-step $k$ of the prediction horizon can then be expressed as:
\begin{subequations}\label{P2}
\begin{equation}\label{eq:P2_obj}
\min\ J
\end{equation}
\begin{equation}\label{eq:P2_ref}
  s.t:\  \eqref{eq:P1_BFM}-\eqref{eq:P1_battery_inv_limit}
\end{equation}
\begin{equation}\label{eq:P2_Pdfix}
    P^{\text{b}}_{n,k}=P^{\text{b}*}
\end{equation}
% \begin{equation}\label{eq:P2_Pcfix}
%     P^{\text{c}}_{n,t}=P^{\text{c}*}
% \end{equation}
\end{subequations}
where $P^{\text{b}*} \in \mathcal{R}^{|\mathcal{P}|}$ are the battery power obtained from the SOCP at node $n$ and time $k$. The NLP given by equations \eqref{eq:P2_obj}-\eqref{eq:P2_Pdfix} is solved separately at each step of the prediction horizon to obtain a feasible plus (near) optimal solution with guaranteed feasibility and a bound on the optimality, as the relaxed SOCP provides a lower bound on the optimal value of the original nonlinear problem.
%~\cite{boyd2004convex}.
Utilizing this SOCP-NLP coupled optimization framework, a scalable solution of three-phase OPF problem can be obtained rapidly, plus the framework provides bounds and guarantees on feasibility and optimality of the solution, where the upper-bound on the global optimality gap is computed from
\begin{equation}\label{eq:opt_gap}
    \text{\% optimality gap} \le \frac{DNLP_{opt}-SOCP_{opt}}{DNLP_{opt}}\times 100.
\end{equation}


\subsection{Linear power-flow model}

In this formulation, the power-flow equations are linearized. {\color{red}[SOUMYA says:] We need to show some plots comparing the results of this linear power-flow based formulation with the SOCP formulation. Question: Should not the solar inverter apparent power constraint in equation (46) include the adjustment due to the solar curtailment $P^{Sc}_{n,k}$\,?}


\begin{align}
% &\min_{P^{\text{b}}_{n,t},q^{\text{b}}_{n,t},S^{\text{S}}_{n,t}}f(x)\label{eq:P1_obj}\\
0=&W_{n,k}-W_{m,k}+(S_{l,k}Z_l^*+Z_lS_{l,k})\ \ \forall l\in \mathcal{L}\label{eq:P1_volt_rel}\\
0=&\text{diag}(S_{l,k}-\sum_{p}S_{p,k})+S^{\text{net}}_{n,k}\ \ \ \forall l\in \mathcal{L}\label{eq:P1_power_balance}\\
0=&\text{real}(S^{\text{net}}_{n,k}-S^{\text{S}}_{n,k}-S^{\text{G}}_{n,k}-S^{\text{b}}_{n,k}+S^{\text{L}}_{n,k})+P^{\text{Sc}}_{n,k}-P^{\text{Lc}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P1_node_real_balance}\\
0=&\text{imag}(S^{\text{net}}_{n,k}-S^{\text{S}}_{n,k}-S^{\text{G}}_{n,k}-S^{\text{b}}_{n,k}+S^{\text{L}}_{n,k})-Q^{\text{Lc}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P1_node_reactive_balance}\\
&|\text{diag}(S_{l,k})|\leq S_{\text{max},l} \qquad \forall l\in \mathcal{L}\label{eq:P1_line_const}\\
&V_{\text{min},n}^2\leq \text{diag}(W_{n,k})\leq V_{\text{max},n}^2 \ \forall n\in \mathcal{N}\label{eq:P1_volt_const}\\
&(\text{real}(S^{\text{S}}_{n,k})-P^{\text{Sc}}_{n,k})^2+\text{imag}(S^{\text{S}}_{n,k})^2|\leq G_{\text{max},n}^2 \qquad \forall n\in \mathcal{N}\label{eq:P1_solar_inv_limit}\\
&|S^{\text{G}}_{n,k}|\leq D_{\text{max},n} \qquad \forall n\in \mathcal{N}\label{eq:P1_diesel_inv_limit}\\
&(P^{\text{b}}_{n,k})^2+(q^{\text{b}}_{n,k})^2\leq H_{\text{max},n}^2, \qquad \forall n\in \mathcal{N}\label{eq:P1_battery_inv_limit}\\
0=&E_{n,k+1}-E_{n,k}+\eta_{\text{b},n}P^{\text{b}}_{n,k}\Delta t \qquad \forall n\in \mathcal{N}\label{eq:P1_battery_power_rel}\\
&E_{\text{min},n}\leq E_{n,k}\leq E_{\text{max},n} \qquad \forall n\in \mathcal{N}\label{eq:P1_SOC_limit}\\
 0\leq & P^{\text{b}}_{n,k}\leq P_{\text{max},n} \qquad \forall n\in \mathcal{N}\label{eq:P1_Pd_limit}
\end{align}

As the power flow equations have been linearized in the above model, this allows us to express the baseline optimization model into the following form:

\begin{align}
    &\min_u f(u)\\
    &\text{s.t.} \ g(x,u)\le 0
\end{align}
where $u$ are the controllable optimization variables which include solar curtailment $P^{\text{Sc}}_{n,k}$, load curtailment $P^{\text{Lc}}_{n,k}$, DG generation $S^{\text{G}}_{n,k}=P^{\text{G}}_{n,k}+jq^{\text{G}}_{n,k}$ and battery output $S^{\text{b}}_{n,k}=P^{\text{b}}_{n,k}+jq^{\text{b}}_{n,k}$. These are the flexible resources available to the microgrid to dispatch in order to meet the load and also satisfy the network constraints (specifically the voltage, line limit and battery state of charge constraints in this case). Furthermore, $x$ represent the dependent optimization variables, such as voltages $W_{n,k}$, line power flows $S_{l,k}$ and battery state of charge (SoC) $E_{n,k}$. These variables cannot be controlled directly, but must satisfy certain constraints given by $g(x,u)$. $f(u)$ represents the objective function that needs to be minimized. In our case, the objective function consists of minimizing the cost of DG generation and minimizing the solar and load curtailment, i.e., 
\begin{align}
    f(u)=\sum_k \sum_n ((a_1 P^{\text{G}}_{n,k}+a_2 P^{\text{Sc}}_{n,k}+a_3 P^{\text{Lc}}_{n,k}+a_4 Q^{\text{Lc}}_{n,k}))
\end{align}

Now with this optimization model we run certain simulation results under different solar and load scenarios shown in the next section 

\subsection{Baseline simulation results}
We provide baseline optimization results under two scenarios: (a) low solar high load (LSHL) and (b) high solar low load (HSLL). The figures below show the generation and load from different sources and the solar and load curtailment, along with the nodal voltages and state of charge. The figures show that the baseline optimization satisfies supply-demand balance and is able to satisfy the voltage and state of charge constraints. Furthermore, the amount of load curtailment is minimum and supply is maintained to critical loads in the system.

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{report_chapters/images/Gen_load_HSLL.png}
\caption{\label{fig:Gen_load_HSLL}Aggregate generation and load.}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:solar_curt_HSLL}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/Solar_curt_HSLL.png}}
    \hfill
  \subfloat [\label{fig:load_curt_HSLL}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/Load_curt_HSLL.png}}
  \caption{Case HSLL: (a) Solar curtailment (b) Load curtailment}
  \label{fig:HSLL_curt}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:volt_HSLL}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/volt_HSLL.png}}
    \hfill
  \subfloat [\label{fig:SoC_HSLL}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/SoC_HSLL.png}}
  \caption{Case HSLL: (a) Nodal voltages (b) Aggregate SoC}
  \label{fig:HSLL_output}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{report_chapters/images/Gen_load_LSHL.png}
\caption{\label{fig:Gen_load_LSHL}Aggregate generation and load.}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:solar_curt_LSHL}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/Solar_curt_LSHL.png}}
    \hfill
  \subfloat [\label{fig:load_curt_LSHL}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/Load_curt_LSHL.png}}
  \caption{Case LSHL: (a) Solar curtailment (b) Load curtailment}
  \label{fig:LSHL_curt}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:volt_LSHL}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/volt_LSHL.png}}
    \hfill
  \subfloat [\label{fig:SoC_LSHL}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/SoC_LSHL.png}}
  \caption{Case LSHL: (a) Nodal voltages (b) Aggregate SoC}
  \label{fig:LSHL_output}
\end{figure}

We also show comparison between the results obtained through the linear power flow model and the SOCP model presented earlier. This comparison is shown in the Fig.~\ref{fig:SOCP_linear_comp} below. From the comparison it can be seen that the results match very closely and this highlights the effectiveness of the linear power flow model to capture the non-linear network model effectively.

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:Linear_LSHL}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/Gen_load_LSHL.png}}
    \hfill
  \subfloat [\label{fig:SOCP_LSHL}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/Gen_load_LSHL_NLP.png}}
  \caption{Case LSHL comparisons: (a) Linear model results (b) SOCP model results}
  \label{fig:SOCP_linear_comp}
\end{figure}

% \begin{itemize}
%     \item \textcolor{red}{Convert this to a multi-stage problem?}
%     \item \textcolor{red}{Inclusion of renewables (perfect forecast?)}
%     \item \textcolor{red}{Inclusion of storage (multi-stage first order DE?)}
%     \item \textcolor{red}{Other inter-temporal constraints for a multi-stage problem? Ramp rate constraints for DG units?}
%     \item \textcolor{red}{This is considering only steady-state operation (no local controls at generator/inverter level) - do we have to include those?}
%     \item \textcolor{red}{Do we consider relaxation-based solution approaches (such as SDP relaxation)?}
% \end{itemize}



==> report_chapters/task2_verification.tex <==
\section{Task 2 Robust Resilience Verification}\label{S:task2_verification}


The goal of this task is to develop algorithms to verify resilience of the closed-loop system (with baseline controls) robustly against a set of adversarial scenarios defined as some bounded sets of events. The adversarial events considered would include, but not limited to, disruptive changes in the system (e.g., loss of significant generation, loss of lines), as well as disruptive failures, malfunctions, or malicious attacks on the sensing, control and communication layers. Resilience specifications would include commonly used industrial surrogate measures such as serviceability of critical loads, and voltage safety (as per ANSI C84.1 Standard); as well as any systems theoretic measures developed within RD2C Thrust 2.1 efforts.

To develop a resilient microgrid optimization framework, we adapt the previously presented optimization model and robustify it against the adversarial events. The main idea behind robustifying the optimization dispatch is to ensure sufficient reserves in generation and curtailment that can respond under the said adversarial events. 

In the most general form the robust optimization problem for a system can be expressed in the following form:
\begin{align}
   & \min_{\textbf{u}} \max_{\textbf{w}} f(\textbf{u},\textbf{w})\\
    s.t. & \ g(\textbf{u},\textbf{x},\textbf{w}) \le 0 \qquad \forall \textbf{w}\in \Omega_W
\end{align}
where $\textbf{u}$ represents the vector of decision variables (generation and curtailment), \textbf{x} represents the vector of dependent optimization variables (voltages and state of charge), $\textbf{w}$ represents the vector of uncertain parameters (outages and data corruption) resulting from the adversarial events and $\Omega_W$ is the finite set in which the adversarial events belong to. The above optimization problem can be converted to a robust formulation using the explicit maximization method~\cite{bai2015robust} in the following form:
\begin{align}
       & \min_{\textbf{u}} \hat{f}(\textbf{u})\\
    s.t. & \ \hat{g}(\textbf{u},\textbf{x}) \le 0 
\end{align}
where $\hat{f}(\textbf{u})=\max_{\textbf{w}} f(\textbf{u},\textbf{w})$ and $\hat{g}(\textbf{u},\textbf{x})=\max_{\textbf{w}} g(\textbf{u},\textbf{x},\textbf{w})$.

% {\color{red}[SOUMYA says:] We need to define $\widehat{f}$ and $\widehat{g}$ clearly. Also, it is not clear what the significance of linearity is in this case. Moreover, there is a third type of variable apart from $x$ (decision variables) and $w$ (uncertain parameters), which refer to the latent optimization variables (e.g., the voltages at nodes).}
The new model does not contain any disturbance terms and if the functions $\hat{f}(\textbf{u})$ and $\hat{g}(\textbf{u},\textbf{x})$ are convex, then the optimization problem is convex, which can be solved efficiently. 

Next we adopt the above robust formulation to the microgrid model presented above.
In order to find the optimal reserve margins required in order to deal with all the adversarial events, we utilize the following robust optimization problem to replace the previously presented deterministic formulation. This robust optimization problem determines the dispatch and reserves of the different flexible resources required to satisfy the network constraints. 

For the microgrid case, the decision variables $\textbf{u}$ are the diesel generator active and reactive power dispatch and reserve amount ($S^{\text{G}}_{n,k}$ and $\Delta S^{\text{G}}_{n,k}$), the battery dispatch and reserve amount ($S^{\text{b}}_{n,k}$ and $\Delta S^{\text{b}}_{n,k}$), the load curtailment and load curtailment reserve ($P^{\text{Lc}}_{n,k}$ and $\Delta P^{\text{Lc}}_{n,k}$, $Q^{\text{Lc}}_{n,k}$ and $\Delta Q^{\text{Lc}}_{n,k}$) and the solar curtailment and solar curtailment reserve ($P^{\text{Sc}}_{n,k}$ and $\Delta P^{\text{Sc}}_{n,k}$).

The disturbance $\textbf{w}$ can be classified into two broad types. The first one arises due to the outage of generating units such as diesel generators, batteries and solar PV units or outage in distribution lines. This is represented by the disturbance in their capacities $S_{\text{max},l}$, $G_{\text{max},n}$, $D_{\text{max},n}$, $H_{\text{max},n}$, $E_{\text{max},n}$ and $P_{\text{max},n}$. The second type of disturbance arises due to the model mismatch in microgrid parameters such as branch impedance values $Z_l$ and battery efficiency $\eta_{\text{b},n}$. 

The goal of the robust microgrid optimization is then to minimize the cost of dispatched generation and reserves while satisfying the device and network constraints for all the disturbances in the selected disturbance set $\Omega_W$. {\color{red}[SOUMYA says:] How is this related to the two goals we mention in Sec.\,2.2? Do we need to use quadratic cost functions, or are linear costs reasonable?} The problem can be formulated as:

\begin{align}
 &\min \sum_k(\sum_n (\alpha_1P^{\text{b}}_{n,k}+\alpha_2 P^{\text{b},\text{R}}_{n,k}+\beta_1P^{\text{Sc}}_{n,k}+\beta_2 P^{\text{Sc},\text{R}}_{n,k}+\gamma_1P^{\text{Lc}}_{n,k}+ \gamma_2 P^{\text{Lc},\text{R}}_{n,k}+\rho_1P^{\text{G}}_{n,k}+\rho_2 P^{\text{G},\text{R}}_{n,k}))\label{eq:P2_obj}\\
  \eqref{eq:P1_volt_rel}&-\eqref{eq:P1_Pd_limit}\\
0=&W^{\text{R}}_{n,k}-W^{\text{R}}_{m,k}+(S^{\text{R}}_{l,k}Z_l^*+Z_lS^{\text{R}}_{l,k})\ \ \forall l\in \mathcal{L}\label{eq:P2_volt_rel}\\
0=&\text{diag}(S^{\text{R}}_{l,k}-\sum_{p}S^{\text{R}}_{p,k})+S^{\text{net},{\text{R}}}_{n,k}\ \ \ \forall l\in \mathcal{L}\label{eq:P2_power_balance}\\
0= &\text{real}( S^{\text{net},{\text{R}}}_{n,k}-S^{\text{S}}_{n,k}(\textbf{w})-S^{\text{G},\text{R}}_{n,k}-S^{\text{b},\text{R}}_{n,k}+S^{\text{L}}_{n,k}(\textbf{w}))+ P^{\text{Sc},\text{R}}_{n,k}-P^{\text{Lc},\text{R}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P2_node_real_balance}\\
0= &\text{imag}( S^{\text{net},\text{R}}_{n,k}-S^{\text{S}}_{n,k}(\textbf{w})-S^{\text{G},\text{R}}_{n,k}-S^{\text{b},\text{R}}_{n,k}+S^{\text{L}}_{n,k}(\textbf{w}))-Q^{\text{Lc},\text{R}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P2_node_reactive_balance}\\
&|\text{diag}(S^{\text{R}}_{l,k})|\leq S_{\text{max},l}(\textbf{w}) \qquad \forall l\in \mathcal{L}\label{eq:P2_line_const}\\
&V_{\text{min},n}^2\leq \text{diag}(W^{\text{R}}_{n,k})\leq V_{\text{max},n}^2 \ \forall n\in \mathcal{N}\label{eq:P2_volt_const}\\
&(\text{real}(S^{\text{S}}_{n,k}(\textbf{w}))-P^{\text{Sc},\text{R}}_{n,k})^2+\text{imag}(S^{\text{S}}_{n,k}(\textbf{w}))^2|\leq (G_{\text{max},n}(\textbf{w}))^2 \qquad \forall n\in \mathcal{N}\label{eq:P2_solar_inv_limit}\\
&|S^{\text{G},
\text{R}}_{n,k}|\leq D_{\text{max},n}(\textbf{w}) \qquad \forall n\in \mathcal{N}\label{eq:P2_diesel_inv_limit}\\
&(P^{\text{b},\text{R}}_{n,k})^2+(q^{\text{b},\text{R}}_{n,k})^2\leq (H_{\text{max},n}(\textbf{w}))^2, \qquad \forall n\in \mathcal{N}\label{eq:P2_battery_inv_limit}\\
0=&E^{\text{R}}_{n,k+1}-E^{\text{R}}_{n,k}+\eta_{\text{b},n}(P^{\text{b},\text{R}}_{n,k})\Delta t \qquad \forall n\in \mathcal{N}\label{eq:P2_battery_power_rel}\\
&E_{\text{min},n}(\textbf{w})\leq E^{\text{R}}_{n,k}\leq E_{\text{max},n}(\textbf{w}) \qquad \forall n\in \mathcal{N}\label{eq:P2_SOC_limit}\\
 0\leq & P^{\text{b},\text{R}}_{n,k}\leq P_{\text{max},n}(\textbf{w}) \qquad \forall n\in \mathcal{N}\label{eq:P2_Pd_limit}
\end{align}
where the terms $W^{\text{R}}_{n,k}$ and $S^{\text{R}}_{l,k}$ are the dependent optimization variables (voltages and line flows) under the disturbance scenarios $(\textbf{w})$, which signify the parameters that are affected by disturbances (namely solar $S^{\text{S}}_{n,k}(\textbf{w})$ and load forecasts $S^{\text{L}}_{n,k}(\textbf{w})$ and generation and line capacities). The controllable optimization variables in this case include the DG generation $S^{\text{G},\text{R}}_{n,k}$, the battery output $S^{\text{b},\text{R}}_{n,k}$, the solar curtailment $P^{\text{Sc},\text{R}}_{n,k}$ and the load curtailment $P^{\text{Lc},
\text{R}}_{n,k}$ and $Q^{\text{Lc},\text{R}}_{n,k}$. These are the generation under the disturbance $\textbf{w}$ and hence the reserve generation can be calculated from their difference from the baseline values, e.g., for DG generation the reserve DG generation is given by: $S^{\text{G},\text{R}}_{n,k}-S^{\text{G}}_{n,k}$. The goal of the optimization is to minimize the cost of the baseline dispatch and reserve amounts, while at the same time ensuring sufficient reserve capability to deal with all adversarial events within the pre-determined disturbance set $\textbf{w}$.

The above optimization problem is intractable as the disturbance set $\textbf{w}$ could be very large. In order to obtain a tractable formulation we reformulate the problem to its robust version by considering the worst-case disturbance. The robust optimization problem can then be expressed as:

\begin{align}
 &\min \sum_k(\sum_n (\alpha_1P^{\text{b}}_{n,k}+\alpha_2 P^{\text{b},\text{R}}_{n,k}+\beta_1P^{\text{Sc}}_{n,k}+\beta_2 P^{\text{Sc},\text{R}}_{n,k}+\gamma_1P^{\text{Lc}}_{n,k}+ \gamma_2 P^{\text{Lc},\text{R}}_{n,k}+\rho_1P^{\text{G}}_{n,k}+\rho_2 P^{\text{G},\text{R}}_{n,k}))\label{eq:P2_obj}\\
  \eqref{eq:P1_volt_rel}&-\eqref{eq:P1_Pd_limit}\\
0=&W^{\text{R}}_{n,k}-W^{\text{R}}_{m,k}+(S^{\text{R}}_{l,k}Z_l^*+Z_lS^{\text{R}}_{l,k})\ \ \forall l\in \mathcal{L}\label{eq:P2_volt_rel}\\
0=&\text{diag}(S^{\text{R}}_{l,k}-\sum_{p}S^{\text{R}}_{p,k})+S^{\text{net},{\text{R}}}_{n,k}\ \ \ \forall l\in \mathcal{L}\label{eq:P2_power_balance}\\
0= &\text{real}( S^{\text{net},{\text{R}}}_{n,k}-S^{\text{S}}_{n,k}(\text{w}^{\text{R}})-S^{\text{G},\text{R}}_{n,k}-S^{\text{b},\text{R}}_{n,k}+S^{\text{L}}_{n,k}(\text{w}^{\text{R}}))+ P^{\text{Sc},\text{R}}_{n,k}-P^{\text{Lc},\text{R}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P2_node_real_balance}\\
0= &\text{imag}( S^{\text{net},\text{R}}_{n,k}-S^{\text{S}}_{n,k}(\text{w}^{\text{R}})-S^{\text{G},\text{R}}_{n,k}-S^{\text{b},\text{R}}_{n,k}+S^{\text{L}}_{n,k}(\textbf{w}))-Q^{\text{Lc},\text{R}}_{n,k} \qquad \forall n\in \mathcal{N}\label{eq:P2_node_reactive_balance}\\
&|\text{diag}(S^{\text{R}}_{l,k})|\leq S_{\text{max},l}(\text{w}^{\text{R}}) \qquad \forall l\in \mathcal{L}\label{eq:P2_line_const}\\
&V_{\text{min},n}^2\leq \text{diag}(W^{\text{R}}_{n,k})\leq V_{\text{max},n}^2 \ \forall n\in \mathcal{N}\label{eq:P2_volt_const}\\
&(\text{real}(S^{\text{S}}_{n,k}(\textbf{w}))-P^{\text{Sc},\text{R}}_{n,k})^2+\text{imag}(S^{\text{S}}_{n,k}(\text{w}^{\text{R}}))^2|\leq (G_{\text{max},n}(\text{w}^{\text{R}}))^2 \qquad \forall n\in \mathcal{N}\label{eq:P2_solar_inv_limit}\\
&|S^{\text{G},
\text{R}}_{n,k}|\leq D_{\text{max},n}(\text{w}^{\text{R}}) \qquad \forall n\in \mathcal{N}\label{eq:P2_diesel_inv_limit}\\
&(P^{\text{b},\text{R}}_{n,k})^2+(q^{\text{b},\text{R}}_{n,k})^2\leq (H_{\text{max},n}(\text{w}^{\text{R}}))^2, \qquad \forall n\in \mathcal{N}\label{eq:P2_battery_inv_limit}\\
0=&E^{\text{R}}_{n,k+1}-E^{\text{R}}_{n,k}+\eta_{\text{b},n}(P^{\text{b},\text{R}}_{n,k})\Delta t \qquad \forall n\in \mathcal{N}\label{eq:P2_battery_power_rel}\\
&E_{\text{min},n}(\text{w}^{\text{R}})\leq E^{\text{R}}_{n,k}\leq E_{\text{max},n}(\text{w}^{\text{R}}) \qquad \forall n\in \mathcal{N}\label{eq:P2_SOC_limit}\\
 0\leq & P^{\text{b},\text{R}}_{n,k}\leq P_{\text{max},n}(\text{w}^{\text{R}}) \qquad \forall n\in \mathcal{N}\label{eq:P2_Pd_limit}
\end{align}
where $\text{w}^{\text{R}}$ denotes the worst-case of the disturbance set $\textbf{w}$. The above optimization problem is deterministic and can be solved efficiently using convex solvers in order to obtain the dispatch and reserve amounts required to counter with the potential disturbances. Furthermore, due to the convex nature of the optimization problem, it has been previously shown in the literature~\cite{liu2017robust} that any disturbance within the set $\textbf{w}$ can be handled with the given reserves provided the extremities of the disturbance set are accounted for, as has been done in the above optimization problem. Later on we will develop a real-time measurement based control algorithm that dispatches reserves in response to measured disturbances. The next sections will also illustrate the effectiveness of the proposed robust formulation through simulation results on IEEE-123 node system. 
\subsection{Real-time reserve control}
In this section we describe a simple measurement based control algorithm that dispatches reserves in response to disturbance events. In microgrids, the amount of flexible generation is increased/decreased based real-time frequency measurements. In our quasi-static analysis, we consider the supply-demand power imbalance to be the measure of frequency and utilize that to dispatch the microgrid reserves in order to meet the demand under disturbance events. Furthermore we employ a simple proportional controller that dispatches reserves in proportion to their available capacity. This can be illustrated by the following equation:
\begin{align}
    Reserve Dispatch=\frac{Reserve Capacity}{Total Reserves}*Imbalance
\end{align}

This control mechanism is utilized in the next section which shows the simulation results. In later analysis we will develop more thorough and sophisticated control algorithms.

\subsection{Robust optimization verification results}

To illustrate the effectiveness of the above presented robust formulation, we consider a disturbance event consisting of a cyber-physical event, wherein a DG trips and become offline and soon after there is a cyber attack which masks the increase in load from the system operator. Considering this event, we solve the optimization problem to dispatch enough generation and maintain sufficient reserves in order to meet the increased demand and also maintain system constraints under this event. The simulation results below illustrate the effective of the robust formulation to deal with this cyber-physical event. 

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:CaseCP_DG_trip}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/CaseCP_DGtrip.png}}
    \hfill
  \subfloat [\label{fig:CaseCP_agg_gen}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/CaseCP_agg_generation.png}}
  \caption{Cyber-physical event case: (a) DG-trip followed by cyber-attack that masks the increase in load (b) Response of the flexible generation and curtailment to deal with this event}
  \label{fig:Case_CP_event}
\end{figure}

\begin{figure}[t]
\centering
\includegraphics[width=0.48\textwidth]{report_chapters/images/CaseCP_reserve.png}
\caption{\label{fig:CaseCP_reserve}Supply demand imbalance created by the cyber-physical event and the reserves available to deal with such an event. The figure shows that enough reserves are available to the system operator to effectively deal with this event.}
\end{figure}

 \begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:CaseCP_SoC}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/CaseCP_SoC_separate.png}}
    \hfill
  \subfloat [\label{fig:CaseCP_volt}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/CaseCP_Volt.png}}
  \caption{Network constraint under cyber-physical event: (a) Battery state of charge (SoC) (b) Network voltages}
  \label{fig:CaseCP_network}
\end{figure}


{\color{red}[Soumya says:] I am not sure if equations (59)-(61) and (67) are correct. The reserves are not actually dispatched, rather are the amounts set aside for use later if/when needed. Thus, the power balance equations in (59)-(61) and (67) should only contain the actually dispatched values, i.e., $S^S_{n,k},S^G_{n,k},S^b_{n,k}$, etc.}

% In order to better understand the robust optimization problem, we reformulate the above optimization into a simpler format and consider the disturbance due to a generator outage. Considering the voltage constraint as an example. Since the above equations are linear, the voltage relation can be expressed as:

% \begin{align}
%     W=M_{\text{p}}(p_{\text{disp}}+\Delta p_{\text{res}}+p_{\text{dist}})+M_{\text{q}}(q_{\text{disp}}+\Delta q_{\text{res}}+q_{\text{dist}})
% \end{align}
% where $W$ is the vector of all the nodal voltages, $p_{\text{disp}}$ and $q_{\text{disp}}$ are the net active and reactive power dispatch from all the flexible resources, $\Delta p_{\text{res}}$ and $\Delta q_{\text{res}}$ are the net active and reactive power reserves from all the flexible resources and $p_{\text{dist}}$ and $q_{\text{dist}}$ are the net active and reactive power disturbance. A robust solution requires that the voltage constraints are satisfied for all values of $(p_{\text{dist}},q_{\text{dist}})\in \Omega_W$. The robust constraints can be expressed by the following two equations:

% \begin{align}
%     M_{\text{p}}(p_{\text{disp}}+\Delta p_{\text{res}}+p_{\text{dist}}^+)+M_{\text{q}}(q_{\text{disp}}+\Delta q_{\text{res}}+q_{\text{dist}}^+)\le V_{\text{max}}\\
%     M_{\text{p}}(p_{\text{disp}}+\Delta p_{\text{res}}+p_{\text{dist}}^-)+M_{\text{q}}(q_{\text{disp}}+\Delta q_{\text{res}}+q_{\text{dist}}^-)\ge V_{\text{min}}\\
% \end{align}
% where $p_{\text{dist}}^+$ and $p_{\text{dist}}^-$ represent the maximum and minimum value of the net disturbance in active generation and similarly for reactive generation. According to the above two equations, the active and reactive power reserves, $\Delta p_{\text{res}}$ and $\Delta q_{\text{res}}$ need to be sufficiently large in order to meet both the extremes of the disturbance set. It can then be shown proved if we are robust to the extreme points of the disturbance set, then we are also robust to the entire disturbance set\cite{liu2017robust}.
\subsection{Robust Resiliency Verification via Dual-Based Approach}
An alternate approach to verifying resiliency is to try and compute the upper bound on the worst-case violation of the resiliency metric for all possible perturbations of the uncertainty set. Let $\Omega_W$ be the uncertainty set and let $R(z)$ be the resiliency metric defined on the optimization decision variables $z \in \mathds{R}^n$ that defines the control law. Let $x \in \mathds{R}^m$ be the set of input parameters that can be subject to adversarial perturbations and the default value of $x$ is $x_{nom}$. In order for resiliency to be satisfied, $R(z) \leq 0$. Then, we can formulate the verification problem for the microgrid as follows:

\begin{align} 
\max_{\omega}~&R(z)\\ \label{eq:verification-1}
s.t~z &= O(x)\\
x &= x_{nom} + \omega\\
\omega &\in \Omega_W\\ \label{eq:verification-n}
\end{align}

The optimization model $O$ for the microgrid model is given by:
\begin{align}
    \min~&\displaystyle\sum_{k=1}^Kc_{0,k}\displaystyle\sum_{\phi\in \mathcal{P}_0} V_{0,k}^{\phi}(I_{0,k}^{\phi})^* + \displaystyle\sum_{k=1}^K\displaystyle\sum_{s\in\mathcal{S}}c_s\displaystyle\sum_{\phi \in \mathcal{P}_s}P_{G,s,k}^{\phi} + \displaystyle\sum_{k=1}^K \displaystyle\sum_{n\in \mathcal{N}\setminus \mathcal{S}} \lambda_{pen,n} \displaystyle\sum_{\phi \in \mathcal{P}_n} P_{c,n,k}^{\phi}\\
    s.t &~(\ref{eq:P1_volt_rel})-(\ref{eq:P1_Pd_limit})
\end{align}

The verification problem posed in (\ref{eq:verification-1})-(\ref{eq:verification-n}) is a bilevel optimization problem that is typically NP-hard. Since the lower-level problem is convex in this case, this problem can be solved by replacing the optimization problem by its KKT (Karush-Kuhn-Tucker) conditions resulting in a MPEC (Mathematical Program with Equilibrium Constraints). It is known that global solution to the MPEC problem is a global solution to the bi-level optimization problem while a local solution might not correspond to a local solution to the bi-level optimization problem. Note that the resulting MPEC is non-convex due to the complementarity conditions which requires the optimal dual variables $\lambda^*$ to be zero or for the corresponding constraints to be binding. In order to solve this problem, we will begin by surveying existing methods presented in \cite{kim2020mpec}. 

The simplest approach to solving the MPEC equivalent verification problem (\ref{eq:verification-1})-(\ref{eq:verification-n}) is to formulate it as an mixed-integer problem. It is known that such models result in large search trees and have weak relaxations. But, since the verification problem only needs to be solved once, it can be done in an offline fashion in a high-performance computing platform.

\subsection{Uncertainty Set Characterization - Inner approximations}
Suppose the constraint set can be expressed as $A [x;\omega] \leq 0$ and $\omega \in \Omega_{w}$. Let $\omega_{nom}$ be the nominal adversarial disturbance and $x_{nom}$ be the corresponding optimal solution. Then, the radius of the largest ball centered at $\omega_{nom}$ that guarantees feasibility of the constraint $A[ x;\omega]$ can be determined by:
\begin{align*}
    &\max_{r,x_i,\omega_i} r\\
    &\omega_i = \omega_{nom} + r e_i~\forall i\\
    &A[x_i;\omega_i] \leq 0 ~\forall i\\
    &\omega_i \in \Omega_w
\end{align*}
where $e_i$ is the i$^\text{th}$ basis vector. The optimal solution to the above problem $x_i^{\star}, \omega_i^{\star}$ will satisfy $A[x_i^{\star}, \omega_i^{\star}] \leq 0$. Then for any convex combination $\omega = \sum_{i=1}^m \beta_i\omega_i^{\star},~\beta_i \geq 0,~\sum_{i=1}^n \beta_i = 1$, we have
\begin{align*}
    A[\sum_{i=1}^m\beta_i x_i^{\star};\sum_{i=1}^m\beta_i \omega_i^{\star}] = \sum_{i=1}^m \beta_i A[x_i^{\star};\omega_i^{\star}] \leq 0.
\end{align*}
This implies any point $\omega$ within the $L_1$ ball centered at $\omega_{nom}$ will be feasible i.e there exists $x$ such that $A[x;\omega] \leq 0$.


\subsection*{ALTERNATE FORMULATION (Soumya)}
Consider the following convex optimization problem parameterized by a disturbance parameter $w \in \mathcal{W}$:
\begin{subequations}
    \begin{align}
    \min_x f(x,w) \\
    s.t~g(x,w) \leq 0
\end{align}
\label{eq:opt0}
\end{subequations}

For a given nominal value of the disturbance $w_{nom}$, the optimal solution $x^\star$ is then given by the KKT conditions:
\begin{align*}
    \mathcal{F}_{nom}(x^\star, w_{nom}) = 0
\end{align*}

The function $\mathcal{F}_{nom}$ which descirbes the KKT conditions is dependent on the binding constraints and remains the same for a specific configuration of binding constraints. If $\mathcal{F}_{nom}$ is continuous, there is a neighborhood $\mathcal{W}_{nom}$ of $w_{nom}$ such that, for every $w_{nom} + \delta w \in {W}_{nom}$, there exists a $\delta x$ such that:
\begin{align*}
    \mathcal{F}_{nom}(x^\star + \delta x, w_{nom} + \delta w) = 0
\end{align*}
A linear approximation of $\delta x$ as function of $\delta w$ can be obtained via Taylor expansion around $x^\star$ and $w_{nom}$. Furthermore, if $\mathcal{F}_{nom}$ is linear, the approximation obtained via Taylor expansion is exact and be expressed via a gain matrix $K$ as:
\begin{align}\label{eq:gain}
    \delta x = K \delta w 
\end{align}

The gain matrix $K$ completely characterizes the change in the optimal solution $x^\star$ \textit{provided the binding constraints do not change}. Note that this provides a conservative estimate of the adversarial perturbations that the system is able to handle. For a given $\delta w$, if (\ref{eq:gain}) has a solution, then the system can handle that perturbation. But if it does not, it either means that the optimization problem given by \eqref{eq:opt0} is infeasible \textit{or} that the set of binding constraints change for that given perturbation.

In case the disturbance $\delta w$ is only partially observable and a low-order linear approximation of the disturbance is given by:
\begin{align*}
    \delta h = H\delta w,
\end{align*}
A linear gain $\bar{K}$ can be constructed by simply solving the following optimization problem:
\begin{align*}
    \min_{\bar{K}} \|K - \bar{K}H \|_{fro}.
\end{align*}
where $\|.\|_{fro}$ is the Frobenius norm.

\section{Cyber Attack Scenarios}

Following are all classified as \emph{Data Integrity Attacks}, which are commonly analyzed in context of modern day power system security research. Some references include: \cite{dehghani2021cyber}, \cite{wang2019deep}, \cite{dehghani2021blockchain}, \cite{sahoo2018stealth}.

\begin{itemize}
    \item \textbf{Injecting measurement errors into PV generation output:} Within this point, we can have several possibilities:
    \begin{itemize}
        \item Inject $\epsilon$ error to the PV generation at all time stamps, i.e.,
        $$\hat{S}_{n,k}^S = S_{n,k}^S\times (1+\epsilon),$$ where $\epsilon \in [-1,1]$. The factor $\epsilon$ can be tweaked to emulated systematic under-estimations as well as over-estimations. For implementation purpose, we can treat $\epsilon$ to be a parameter, and vary in discrete steps, such as $\epsilon = \{0.1, 0.2, 0.3\}$. 
        \item Inject time-varying errors instead of static error (given in earlier point). 
    \end{itemize}
    This type of error, left untreated, can lead to ramp-induced attacks (RID), as discussed in details in \cite{che2019impact}.
    
    \item \textbf{Injecting latency to PV generation output measurement (Replay attack):} In this type of attack (see, for example \cite{habibi2020detection}), the measured PV-generation output is maliciously changed to reflect the true generation at a previous time stamp (with $\delta$ delay). Mathematically, $$\hat{S}_{n,k}^S = S_{n,k-\delta}^S,$$ where $\hat{S}^S$ denotes the measured PV-generation output to be used in the microgrid optimization.
    
    \item \textbf{Injecting errors to load measurement (corrupted state estimation):} This type of attack is also known as load curtailment cyber-attack (see \cite{kushal2018risk}, \cite{banerjee2021online} for detailed case studies). Similar to generation setpoint change attack, assuming $\epsilon$ to be the malicious error injection, we can write:
    $$ \hat{S}_{n,k}^L = S_{n,k}^L \times (1 + \epsilon), $$
    Note that as given in \cite{kushal2018risk}, it may be optimal for the attacker (causing maximal disruption) when this type of attack is initiated around afternoon (12 pm) and continued till peak evening hours. 
    
    \item \textbf{Partial/complete loss of dispatchable generation capability:}
    
    \item \textbf{Coordinated attack schemes:} In this type of attack, the attacker often has access to multiple critical information of the system, and is in a position to maliciously pose threats in a coordinated manner, from multiple sources. Please see the following references for examples of such attacks, which often include attacks in both the cyber as well as the physical layer: \cite{sun2018cyber}, \cite{he2021tri}, \cite{che2019impact}. In our work, we consider at least 1 type of coordinated attack scheme, where the attacker can simultaneously inject error signals to load estimation as well as PV-forecast, such that load is under-estimated and PV-generation is over-estimated, so that the real time generation-load imbalance is magnified, thus upsetting real time grid operations.
\end{itemize}

\section{Chance constrained optimization}
The focus of this task will be to develop chance constrained formulations for the resilient optimization problem. We will develop risk based algorithms for resilience verification using measures such as Value at Risk (VaR), conditional value at risk (cVaR) and measures to address high-impact low-probability (HILP) events. 

\subsection{Motivation for chance constraints}
Robust optimization techniques can be overly conservative as they consider the worst case of the disturbance. Some of these disturbances or adversarial events can have a very low probability of occurrence, which is not accounted for in the robust method. As a result, solutions obtained through robust optimization can be overly conservative and in the worst-case even infeasible, i.e., no solution can guarantee satisfaction of constraints under all the different disturbances. In order to avoid this situation, it becomes necessary to consider the probability distribution of the different disturbance events and their impact level on the system. This can especially help us in being resilient to high-impact low-probability events. Chance constrained based methods guarantee system constraints with a high but given probability level, that can be acceptable to the system operator. This way we avoid being unnecessarily robust to events that have very low probability of occurrence. 

\subsection{Chance constraint technical summary}
In chance constraint formulations, we want our solution to be resilient with some probability. 

In the most general form the stochastic optimization problem for a system can be expressed in the following form:
\begin{align}
   & \min_{\textbf{u}} f(\textbf{u},\textbf{w})\\
    s.t. & \ g(\textbf{u},\textbf{x},\textbf{w}) \le 0 \qquad \forall \textbf{w}\in \Omega_W
\end{align}
where $\textbf{u}$ represents the vector of decision variables (generation and curtailment), \textbf{x} represents the vector of dependent optimization variables (voltages and state of charge), $\textbf{w}$ represents the vector of uncertain parameters (outages and data corruption) resulting from the adversarial events and $\Omega_W$ is the finite set in which the adversarial events belong to. Previously, the above stochastic problem has been solved through robust optimization by considering the worst case of the adversarial events. In this section we shall consider the chance constraint formulation as shown below:

\begin{align}
   & \min_{\textbf{u}}\mathbb{E}[ f(\textbf{u},\textbf{w})]\\
    s.t. & \ \mathbb{P}[g(\textbf{u},\textbf{x},\textbf{w}) \le 0] \ge 1-\alpha \qquad \textbf{w}\in \Omega_W
\end{align}

where $\alpha$ is the acceptable violation level, which can be chosen by the system operator according to his specifications. 

In the microgrid application, we require to choose our dispatch and reserve in such a way that the chance constraints are satisfied, i.e., 

\begin{align}
    R^-_{n,k}\le P_{n,k}\le \overline{S}_{n,k}-R^+_{n,k}
\end{align}
where $P_{n,k}$ is the active power dispatch, $R^-_{n,k}$ is the down reserve, $R^+_{n,k}$ is the up-reserve and $\overline{S}_{n,k}$ is the device power limit at node $n$ and time $k$. 
An example of a constraint that needs to be satisfied is that there need to be sufficient up-reserves available in order to deal with any loss of generation. As a chance constraint, this can be expressed at each time-step as:

\begin{align}
    \mathbb{P}[\sum_nR^+_{n,k}+A\textbf{w}\ge 0] 1-\alpha
\end{align}

The above constraint is stochastic in nature and hence makes the optimization problem intractable. Depending upon the nature of the underlying distributions, there exists many reformulations in the literature to convert the above stochastic formulation into a tractable deterministic formulation, while satisfying the constraints. One is such reformulation is given below:

\begin{align}
    \sum_nR^+_{n,k}+\phi^{-1}(1-\alpha)||A\Sigma_w^{1/2}||_2\ge 0
\end{align}

where $\phi^{-1}(1-\alpha)$ is the safety factor and can be calculated depending upon the type of the distribution. For example, closed form solutions exist for the safety factor, when the distribution is either uniform or Gaussian. Furthermore, if the mean and variance of the distribution are known, a Chebyshev reformulation can provide a value for the safety factor, however, it may be very conservative. The next section provides simulation results when the uncertainty distribution is assumed to be Gaussian. 

Future work will consider the distributionally robust chance constraint using Wasserstein ambiguity sets, multi-modal distributions and also differentiate been VaR and cVaR based methods. We will further look into chance constraints for rare events, i.e., events will probability less than $10^{-6}$. We will also look into combining different probability distributions of different disturbances within a single system response. 

\subsection{Chance constraint simulation results}
Simulations results were conducted on the modified IEEE-123 node system. In this case we assumed the solar and load forecasts to be uncertain and belonging to a Gaussian distribution with known mean and variance as shown in Fig.~\ref{fig:solar_Gaus} and Fig.~\ref{fig:load_Gaus}. We apply the above chance constraint formulation for Gaussian distributions with $\alpha = 0.05$ (i.e., we would like the constraints to be satisfied atleast 95\% of the time). 


\begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:solar_Gaus}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/solar_dist.png}}
    \hfill
  \subfloat [\label{fig:load_Gaus}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/load_dist.png}}
  \caption{(a) Solar forecast error distribution (b) Load forecast error distribution}
  \label{fig:Gaus_dist}
\end{figure}

Fig.~\ref{fig:CC_time} shows the disturbance values along with the available up and down reserves to account for the disturbances over time. As can be seen from the figure, more than 95\% of the time, there are enough reserves to account for the forecast error. This is further illustrated by Fig.~\ref{fig:CC_hist} , which shows a histogram of all the forecast errors, with blue being accounted for through reserves and red being not. As can be seen more than 95\% of forecast errors are being accounted for through the reserves calculated using the chance constraint formulation.

\begin{figure}[t]
    %\centering
    \vspace{-9pt}
  \subfloat [\label{fig:CC_time}]{   \includegraphics[width=0.46\textwidth]{report_chapters/images/CC_gaussian_balance.png}}
    \hfill
  \subfloat [\label{fig:CC_hist}]{    \includegraphics[width=0.46\textwidth]{report_chapters/images/CC_gaussian_dist.png}}
  \caption{(a) Comparison of the up and down reserves with the disturbance over time (b) Distribution of the forecast error showing that more than 95\% of the disturbances (in blue) as within the reserve margins and hence accounted for.}
  \label{fig:CC_balance}
\end{figure}

\section{Distributionally robust optimization (DR)}
\subsection{Wasserstein metric based DR optimization}
Consider the distributionally robust chance constrained optimization problem:
\begin{align}
    \min_x \sup_{\mathbb{P} \in \hat{P_N}} \mathbb{E}_{\mathbb{P}}{f(x,\zeta)}\\
    \text{s.t} \ \inf_{\mathbb{P}\in \hat{P_N}}\mathbb{P}[g(x,\zeta)\le 0]\ge 1-\rho
\end{align}

where $x\in \mathbb{R}^p$ is the decision variable, $\zeta\in \mathbb{R}^m$ is the uncertain random variable belonging to the ambiguity set $\hat{P_N}$ of probability distribution constructed from the available historical data $\mathbb{\hat{P_N}}$, i.e., $\mathbb{\hat{P_N}}=\frac{1}{N}\sum_{k=1}^N\delta_{\hat{\zeta}^{(k)}}$ and where the historical samples are given by: $\{\hat{\zeta}^{(1)}, \hat{\zeta}^{(1)}, \hdots, \hat{\zeta}^{(N)}\}$ and $\hat{\zeta}\in \mathbb{R}^m$ and $\rho$ is the chosen confidence level.\\

$\hat{P_N}$ is the Wasserstein ball of radius $\epsilon(N)$ centered at the emperical distribution $\mathbb{\hat{P_N}}$, i.e., 
\begin{align}
    \hat{P_N}=\{\mathbb{P}\in P(\Omega): W(\mathbb{P}, \mathbb{\hat{P_N}} < \epsilon(N)\}
\end{align}
where the Wasserstein radius is given by:
\begin{align}
    \epsilon(N)=C\sqrt{\frac{1}{N}log(\frac{1}{\rho})}
\end{align}
and the Wasserstein metric between marginal distributions $\mathbb{Q}_1$, $\mathbb{Q}_2$ $\in P(\Omega)$ is given by:
\begin{align}
    W(\mathbb{Q}_1,\mathbb{Q}_2)=\inf_{\pi}\{\int_{\Omega^2}||\zeta_1-\zeta_2||\pi(d\zeta_1,d\zeta_2)\}
\end{align}
where $\pi$ is the joint distribution of $\zeta_1$ and $\zeta_2$.\\
In the expression of $\epsilon(N)$, the value of $C$ can be obtained from solving the following optimization problem:
\begin{align}
    C\approx 2 \inf_{\alpha >0}(\frac{1}{2\alpha}(1+\ln(\frac{1}{N}\sum_{k=1}^Ne^{\alpha||\hat{\zeta}^{(k)}-\hat{\mu}||_1^2})))^{1/2}
\end{align}
where the above minimization over $\alpha$ is solved using the bisection search method and $\hat{\mu}$ is the sample mean.\\
The above chance constraint is equivalent to finding finding a set $\mathbf{U}$ s.t.
\begin{align}
    g(x,\zeta)\le 0, \ \forall \zeta \in \mathbf{U}
\end{align}
Construct a new sample set $v$, s.t.
\begin{align}
    v=\hat{\Sigma}^{-1/2}(\zeta-\hat{mu})
\end{align}
Now the chance constraint is reformulated as:
\begin{align}
    \sup_{\mathbb{Q}\in \hat{Q_N}}\mathbb{Q}[v \notin \mathbf{V}]\le \rho
\end{align}
where the set $\mathbf{V}$ is given by:
\begin{align}
    \mathbf{V}(\sigma)=\{v\in \mathbb{R}^m | -\sigma \mathbf{1}<v<\sigma\mathbf{1}\}
\end{align}
where $\sigma$ is obtained by solving the following optimization problem:
\begin{align}
    \min_{0\le \lambda, 0\le \sigma \le \sigma_{\max}} \sigma \text{s.t} \ h(\sigma,\lambda) \le \rho
\end{align}
where 
\begin{align}
    h(\sigma,\lambda)=\lambda\epsilon +\frac{1}{N}\sum_{k=1}^N(1-\lambda(\sigma-||\hat{v}^{(k)}||_{\infty})^+)^+
\end{align}
The above optimization problem can again be solved with the bisection search method. Based on the obtained value of $\sigma$, the set $\mathbf{V}$ can be obtained as:
\begin{align}
    \mathbf{V}(\sigma)=conv(\{\pm \sigma,\pm \sigma\})
\end{align}
which then based on the transformation $u^{(i)}=\hat{\Sigma}^{1/2}v^{(i)}+\hat{\mu}$ results in the following set $\mathbf{U}$
\begin{align}
    \mathbf{U}=conv(\{u^{(1)},u^{(2)}, \hdots, u^{(2^m)}\})
\end{align}
which then results in the following distributionally robust constraint:
\begin{align}
    g(x,u^{(i)})\le 0, \ 1\le i\le 2^m
\end{align}
which is a convex constraint and can be solved in a scalable manner.

==> report_chapters/task3_adaptation.tex <==
\section{Task 3 Resilient Control Adaptation}\label{S:task3_adaptation}

The goal of this task is to design adaptive control strategies that assure resilience of the closed-loop system against a set of adversarial scenarios. Specific approaches considered would include proactive tuning of the baseline controller settings (parameters) using techniques from robust nonlinear optimization [6], as well as online adaptation of the baseline control solution via various gradient-based approaches [2-3]. Pareto fronts of co-optimality would be used to demonstrate the trade-offs between resilience and other baseline control objectives (such as, efficiency).

\subsection{Approach (subject to change)}
Suppose $\textbf{u}^\star$ is the optimal dispatch associated with the baseline optimization problem and $\Delta \textbf{u}^\star$ be the available reserves. For a given realization of the disturbance $w$, we can calculate the margins $c(w)$ as follows:
\begin{align}
    c(w) = g(\textbf{u}^\star, w)
\end{align}
If the constraints are satisfied, then $c(w) \leq 0$.

The optimal reserve dispatch problem can then be formulated as a function of the constraint violations $c(w)$ as follows:

\begin{align}
    \textbf{K}_i = &\max_{w_i, k} \alpha_i\\
    &g(\mathbf{u}^* + \delta u, w_i) \leq 0\\
    &\delta u \leq \Delta \mathbf{u}^*\\
    &\delta u = k^T c(w_i)\\
    &w_i = w^{nom} + \alpha_i e_i\\
    &w_i \in \Omega_w
\end{align}



==> report_chapters/task4_codesign.tex <==
\section{Task 4 Co-Design Use-Case}\label{S:task3_adaptation}

The goal of this task is to generate a technical summary report discussing the co-design problem and its various methodologies in general, and then present one (or more) specific use-case problem centered around ALERT.
